Size-effects of metamaterial beams subjected to pure bending: on boundary conditions and parameter identification in the relaxed micromorphic model

In this paper we model the size-effects of metamaterial beams under bending with the aid of the relaxed micromorphic continuum. We analyze first the size-dependent bending stiffness of heterogeneous fully discretized metamaterial beams subjected to pure bending loads. Two equivalent loading schemes are introduced which lead to a constant moment along the beam length with no shear force. The relaxed micromorphic model is employed then to retrieve the size-effects. We present a procedure for the determination of the material parameters of the relaxed micromorphic model based on the fact that the model operates between two well-defined scales. These scales are given by linear elasticity with micro and macro elasticity tensors which bound the relaxed micromorphic continuum from above and below, respectively. The micro elasticity tensor is specified as the maximum possible stiffness that is exhibited by the assumed metamaterial while the macro elasticity tensor is given by standard periodic first-order homogenization. For the identification of the micro elasticity tensor, two different approaches are shown which rely on affine and non-affine Dirichlet boundary conditions of candidate unit cell variants with the possible stiffest response. The consistent coupling condition is shown to allow the model to act on the whole intended range between macro and micro elasticity tensors for both loading cases. We fit the relaxed micromorphic model against the fully resolved metamaterial solution by controlling the curvature magnitude after linking it with the specimen's size. The obtained parameters of the relaxed micromorphic model are tested for two additional loading scenarios.

==> conclusions_sec.tex <==
%=========================================================================
\sect{\hspace{-5mm}. Conclusions}
\label{sec:con}
We introduced the relaxed micromorphic model with standard and modified mixed formulations and presented the main aspects related to the construction of a $H^1(\B) \times H(\curl,\B) \times H^1(\B)$ finite element for the mixed formulation. We investigated for a force-driven problem the behavior of  the relaxed micromorphic model for two cases. The relaxed micormorphic model exhibit undesired behavior when the consistent boundary condition was enforced on the displacement's Dirichlet boundary  where no size-effect were captured and linear elasticity with $\Cmacro$ was reproduced for any value of the characteristic length. The important role of the characteristic length was restored and the expected behavior of the relaxed micromorphic model was noticed when the consistent boundary condition was enforced on the whole boundary. A drawback of enforcing the consistent boundary condition on the whole boundary is building a boundary layer for small values of characteristic length which demand finer mesh to be resolved. Finally, we investigated the different stress measurements of the relaxed micromorphic model. An interesting finding is that the micro-stress transfers the traction vector on the boundary for any values of the characteristic length.
\vspace{2 cm}

{\bf Acknowledgement} \\
Funded by the Deutsche Forschungsgemeinschaft (DFG, German research Foundation) -  Project number 440935806 (SCHR 570/39-1, SCHE 2134/1-1, NE 902/10-1) within the DFG priority program 2256. The authors gratefully acknowledge Jo\v{z}e Korelc for the development and ongoing support when using AceGen and AceFEM.




%=========================================================================
 


==> fgeneralized_continua_01.tex <==

%========================================================================
%          ***  First Page of Paper  ***
%========================================================================
\thispagestyle{empty}

% \ce{{\Large UNIVERSITY OF DUISBURG ESSEN}
% \phantom{x}
% {\large CAMPUS ESSEN}}

\phantom{X\hfill X}

\unitlength1cm
\begin{picture}(14,6.85)
\put(0,5){\includegraphics[width=6.0cm]{logo_claim_4c.eps}}
\put(13.3,5){\scalebox{0.405}{\includegraphics{penrose_color_new.eps}}}
% \put(7.0,1.95){\scalebox{0.40}{\input{penrose_color.pstex_t}}}
\put(7,5){\parbox[b]{8cm}{%
\definecolor{udeblue}{cmyk}{1,0.68,0.0,0.12}
\sffamily\color{black}%
Universit\"at Duisburg-Essen\\
Institut f\"ur Mechanik\\
Fakult\"at f\"ur Ingenieurwissenschaften\\
Abteilung Bauwissenschaften\\
Prof. Dr.-Ing. J. Schr\"oder
}}
\end{picture}

\vspace*{-2cm}

\begin{center}

\begin{Huge}
\bfseries%
\end{Huge} 
\medskip

\begin{large}
\bfseries%
Size-effects of metamaterial beams subjected to pure bending: on boundary conditions and parameter identification in the relaxed micromorphic model
\end{large}

\vspace{1.0cm}

{\large by Mohammad Sarhil, Lisa Scheunemann, J\"org Schr\"oder and   \\ Patrizio Neff}

\vspace{1.0cm}

type of report:\\
Manuscript under construction

\vspace{0.5cm}

submitted to \\
\textit{XXX}\\
on Month Day, Year

\vfill

{\bfseries\tabcolsep3mm\renewcommand{\arraystretch}{1.5}%
\begin{tabular}{|c|c|}
\hline
Report - Preprint & No. XX\\
\hline
\end{tabular}}


\vspace{.2cm}
Tag. Monat Jahr  % Tag der finalen Version 

\vspace{0.6cm}
% Versionsdatum, in der finalen Version auskommentieren!!!
Version: {\bfseries\textcolor{red}\today} 

\vspace{0.6cm}

Editor: Prof. Dr.-Ing. habil. J\"org Schr\"oder

\vspace{0.cm}
{Universit\"atsstra\ss e 15, 45141 Essen, Germany}

\end{center}

\newpage



==> relaxed_bending_sec.tex <==
{\color{blue}
\sect{\hspace{-5mm}. Relaxed micromorphic model for a beam subjected to bending}
We use a beam with dimensions $2\times 1$ and the following material parameters for the relaxed micromorphic model. 
\begin{table}[ht]
\center
\begin{tabular}{|c|}
\hline
$\mu_e = \mu_\textrm{micro}  = 1$, \\
 $  \lambda_e = \lambda_\textrm{micro} = 1$, \\
$\mu_\textrm{c} = 0 $,  
$\kappa_2 = 10^3 (1+\Lc^2)$ \\
 $\Lc$ varies for all cases\\
\hline
\end{tabular}
\caption{Material parameters of the relaxed micromorphic model.}
\end{table}
\subsection{First and second tests}
The boundary value problems are shown in Figures  	\ref{Fig:test1-r_geo} and \ref{Fig:test2-r_geo}. 
Relaxed micromorphic model captures successfully the size-effects,  see Figure \ref{Fig:test1+2_energy}, and the solution is the same for both boundary value problems. We notice that the  displacement nodes on right edge has zero reaction forces for big values of $\Lc$ and  the  micro-distortion nodes on the right edge has zero reaction forces for small values of $\Lc$. 
\begin{figure}[ht]
\center
	\unitlength=1mm
	\begin{picture}(130,60)
	\put(0,0){\def\svgwidth{11 cm}{\small\input{figures/test1_geo.eps_tex}}}
       \put(12.115090838,30.30393048){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{\scriptsize $\Bdis \cdot \Btau =(+ \kappa l /2,0)^T$}}}%
       \put(74.115090838,30.30393048){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{\scriptsize $\Bdis \cdot \Btau =(- \kappa l /2,0)^T$}}}%
	\end{picture}
	\caption{Boundary value problem of first test using relaxed micromorphic model. }
	\label{Fig:test1-r_geo}
\end{figure} 

\begin{figure}[ht]
\center
	\unitlength=1mm
	\begin{picture}(60,60)
	\put(0,0){\def\svgwidth{5.5 cm}{\small\input{figures/test2_geo.eps_tex}}}
       \put(55.115090838,23.30393048){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{\scriptsize $\Bdis \cdot \Btau =(- \kappa l /2,0)^T$}}}%
         \put(10.115090838,20.30393048){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{\scriptsize $(\Bdis \cdot \Btau)_x = 0 $}}}%
	\end{picture}
	\caption{Boundary value problem of second test using relaxed micromorphic model. }
	\label{Fig:test2-r_geo}
\end{figure} 

\begin{figure}[ht]
\center
	\unitlength=1mm
	\begin{picture}(120,90)
    \put(0,0){\includegraphics[width=12 cm]{figures/Rizzi_bending.eps}}%
	\end{picture}
	\caption{Total energy varying $\Lc$. Using gradient of the micro-distortion field leads to unbounded stiffness for small sizes. }
	\label{Fig:test1+2_energy}
\end{figure} 
\FloatBarrier
\subsection{Third test}

\begin{figure}[ht]
\center
	\unitlength=1mm
	\begin{picture}(60,60)
	\put(0,0){\def\svgwidth{8 cm}{\small\input{figures/test3_geo.eps_tex}}}
 \put(13.264771,22.782009){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$(\Bdis \cdot \Btau)_x =0$}}}%
  \put(35.0264771,47.2782009){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$(\Bdis \cdot \Btau)_y =0$}}}%
	\end{picture}
	\caption{Boundary value problem for the third test. }
		\label{Fig:test3_geo}
\end{figure} 

The relaxed micromorphic model show no size-effects.  

\textrm{Ideas} \\
1) Spiting the applied moment right to two moments 
\begin{equation}
\bM = f(\Lc) \bM_u +  (1- f(\Lc)) \bM_\dis
\end{equation}
where  $f(\Lc) \in [0,1]$. \\
2)  Applying the consistent boundary condition right by using the penalty method: certainty shows size-effect. 

}
\FloatBarrier

==> sec_all.tex <==
%%%
%%% Geodesic FEM
%%%


\thispagestyle{empty}
\ce{\bf \large
Relaxed Micromorphic Continua 
}

\vspace{2mm}
\ce{\bf 
Lagrange-type  versus $H(\curl,\B)$ FEM realization - a first study 
}

%\medskip
%\ce{\bf \large
%porous magneto-electric two-phase composites
%}

% % % \vspace{-3mm}
% % % \begin{center}
% % % {\bf \large
% % % FE${}^2$-scheme: Localization and Homogenization.
% % % }
% % % \end{center}

\vspace{4mm}
\ce{J. Schr\"oder$^\ast $, M. Sarhil, L. Scheunemann \& P. Neff}

\vspace{4mm}
\ce{$^1$Institute of Mechanics, University of Duisburg-Essen}
\ce{Universit\"atsstr. 15, 45141 Essen, Germany}
\ce{\small e-mail: 
j.schroeder@uni-due.de
}    

\vspace{4mm}
\ce{$^2$Institute of Mathematics, University of Duisburg-Essen,}
\ce{ 45141 Essen, Germany,}
%\ce{\small e-mail: 
%j.schroeder@uni-due.de
%}    


    
\vspace{4mm}
\begin{center}
{\bf \large Abstract}
\bigskip

{\footnotesize
\begin{minipage}{14.5cm}
\noindent
In this contribution, we discuss the convergence behavior of Lagrange-type and edge-based finite element discretizations for the so-called relaxed micromorphic continua. 
\end{minipage}
}
\end{center}

{\bf Keywords:} 
Relaxed Micromorphic Model,
Finite Elements,
...
etc.


%=========================================================================
\sect{\hspace{-5mm}. Introduction}
\vspace{-4mm}
%=========================================================================
The recent advances of  the additive manufacturing (AM, or 3D printing) techniques are empowering the fabrication process of the three-dimensional architected  metamaterials, c.f. \cite{JiaLi:2018:3pa,MonKuaArnQi:2020:rai,PloPan:2019:rod,LeiHonZhaHamCheLuQi:2019:3po}.  Metamaterials are receiving tremendous attention in both academia and industry due to their unconventional mechanical properties which are not solely governed by the bulk mechanical properties but also by the geometry of the unit cells which can be designed to attain the desired functionality, see \cite{FisHilEbe:2020:mmo,LeeSinTho:2012:mnm,SurGaoDuLiXioFanLu:2019:AEM,YaZhoLiaJiaWu:2018:mma,Zad:2016:mmm}.  To simply the design process of novel metamaterials, suitable computational tools are needed to obtain their unprecedented effective mechanical properties. The classical Cauchy-Boltzmann theory and the first-order homogenization procedures fail to describe the mechanical macroscopic behavior of mechanical metamaterials since they exhibit the size effect phenomenon, e.g. small specimen are stiffer than the big specimen, and therefore other generalized theories are needed such as the classical Mindlin-Eringen micromorphic theory, c.f. \cite{Min:1964:msi,SuhEri:1964:nto,EriSub:1964:nto,Eri:1968:mom}, Cosserat theory, \cite{CosCos:1909:tof}, gradient elasticity,  \cite{MinEsh:1968:ofsg,AltAif:1997:osa,FisKlaMerSteMue:2011:iao}, or others. 

The relaxed micromorphic model recently  which we adopt in this work is introduced in \cite{NefGhiMadPlaRos:2014:aup,GhiNefMadPlaRos:2015:trl,NefGhiLazMad:2015:trl}. It keeps the full kinematics of the  micromorphic theory but employs the matrix Curl operator of a non-symmetric second-order micro-distortion field for the curvature measurement.  The relaxed micromorphic model reduces the complexity of the classical micromorphic theroy by reducing the material parameters and has shown many advantages such the bounded stiffness for very small sizes.  Furthermore, it has already used to obtain the main mechanical characteristics (stiffness, anisotropy, dispersion) of the targeted metamaterials for many well-posed dynamic and static problems, e.g. \cite{MadNefGhiPlaRos:2015:bgi,MadNefGhiPlaRos:2015:wpi,MadNefGhiRos:2016:rat,MadNefBar:2016:cbg,NefMadBarDagAbrGhi:2017:rwp,BarMadDagAbrGhiNef:2017:taf,MadNefBarGhi:2017:aro,MadColMinBilOuiNef:2018:mpc,BarTalDagAivNefMad:2019:rmm,AivTalAgoDaoNefMad:2020:fan}. Recently, the scale independent short range elastic parameters in the relaxed micromorphic model were determined for given periodic microstructures in \cite{NefEidMad:2019:ios} which used to capture the band-gaps as  a dynamical property of the targeted mechanical metamaterial in \cite{DagBarGhiEidNefMad:2020:edo}.  The analytical solutions of the relaxed micromorphic compared to solutions of other generalized continua for simple boundary value problems, i.e. shear, bending, torsion and uniaxial tension, are discussed in \cite{RizHueKhaGhiMadNef:2021:aso1,RizKhaGhiMadNef:2021:aso2,RizHueMadNef:2021:aso3,RizHueMadNef:2021:aso4}. 

Because of using the Curl matrix operator of the micro-distortion for the curvature measurement, the relaxed micromorphic model seeks the solution of the micro-distortion in $H(\curl)$ space while the macroscopic displacement solution is still in $H^1$ space.  The appropriate finite elements of such case must be conforming in $H(\curl)$ space. Edge-based finite elements were firstly discussed by \cite{Whi:1957:git}.  The 2D formulation of $H(\div)$-conforming elements was presented first in \cite{RavTho:1977:amf}. In \cite{Ned:1980:mfe,Ned:1986:anf}  $H(\curl)$-conforming tetrahedral and brick elements were first introduced.  An extension to elements with curved edges, based on covariant projections, was developed by \cite{CroSilHur:1988:cpe}. A detail review about the $H(\div)$- and $H(\curl)$-conforming finite elements is available in \cite{KirLogRogTer:2012:cau} and \cite{RogKirAnd:2009:eao}. 
A mixed $H^1 \times H(\curl)$ finite element formulation for a simplified anti-plane shear case of the relaxed micromorphic model utilizing a scalar displacement and a vectorial micro-distortion is available in \cite{SkyNeuMueSchNef:2021:CM}.



\clearpage
%=========================================================================
\sect{\hspace{-5mm}. Relaxed Micromorphic Model}
\vspace{-4mm}
%=========================================================================

The relaxed micromorphic model is a continuum model describes the kinematics of a material point using a displacement vector $\bu\colon\Omega\subseteq\R^3\to\R^3$ and a non-symmetric micro-distortion field  $\Bdis\colon\Omega\subseteq\R^3\to\R^{3\times3}$. Both are defined by the following potential minimization for the static case 
\begin{equation}
\label{eq:pot}
\Pi = \int_\Omega W\left(\nabla \bu,\Bdis,\curl \Bdis \right) \, - {\bbf}\cdot{\bu} \, - \bM : \Bchi \,\textrm{d}V\ - \int_{\partial \Omega} \bt^u \cdot \bu  \,\textrm{d}A  - \int_{\partial \Omega} \bT^\chi : \Bchi  \,\textrm{d}A  \longrightarrow\ \min\,,
\end{equation}
with $(\bu,\Bchi)\in H^1(\Omega)\times H(\curl,\Omega)$. The vector $\bbf \in L^2$ and the tensor $\bM$ describe, respectively, the body force and the body moment, while $\bt^u$ and $\bT^\chi$ are the traction vector and double traction tensor. The elastic energy $W$ reads  
\begin{equation}
\begin{array}{rl}\displaystyle
W &= \displaystyle \dfrac{1}{2}
 \left( \right.
\underbrace{\symb{ \nabla \bu - \Bchi} : \Ce : \symb{ \nabla \bu - \Bchi} }_{\textrm{anisortropic elastic energy}}
 + \underbrace{\sym \Bchi : \Cmicro: \sym \Bchi}_{\textrm{micro energy}}
\\[3mm]
&+ \underbrace{\skewb{ \nabla \bu - \Bchi} : \Cc : \skewb{ \nabla \bu - \Bchi}}_{\textrm{anisotropic rotational elastic coupling}}
 + \underbrace{\mu \, \Lc^2 \, \textrm{Curl} \Bchi : \IL :\textrm{Curl} \Bchi}_{\textrm{curvature}} \left. \right)\,.
\end{array}
\label{eq:potential}
\end{equation}
Here, $\Cmicro,\Ce$ are fourth order positive definite stadnard elasticity tensors, $\Cc$ is a fourth order positive semi-definite rotational coupling tensor, $\IL$ is a scale-dependent fourth-order tensor, $Lc$ is a non-negative characteristic length scale, $\mu$ is a typical shear modulus.   The relaxed micromorphic model employs the curl of micro-distortion field for the curvature measurement resulting in many advantages such as the bounded stiffness for the small-size samples. 

The variation of the potential with respect to the displacement field leads to
\begin{equation}
\delta_{\bu} \Pi =  \int_{\Omega} \{ \Ce : \symb{ \nabla \bu - \Bchi}+  \Cc : \skewb{ \nabla \bu - \Bchi} \} :  {\nabla \delta \bu}  -  \bbf \cdot \delta \bu \, \textrm{d}V - \int_{\partial \Omega} \bt^u \cdot \delta \bu  \,\textrm{d}A = 0,
\end{equation} 
which can be formulated using integration by parts and divergence theorem as 
\begin{equation}
\begin{aligned}
\delta_{\bu} \Pi = &  - \int_{\Omega}  \{ \Divb{\Ce : \symb{ \nabla \bu - \Bchi} + \Cc : \skewb{ \nabla \bu - \Bchi}} + \bbf \} \cdot \delta \bu \, \textrm{d}V \\ &- \int_{\partial \Omega} \{ \bt^u - \{ \Ce : \symb{ \nabla \bu - \Bchi} + \Cc : \skewb{ \nabla \bu - \Bchi} \} \cdot \bn \} \cdot \delta \bu  \,\textrm{d}A = 0,
\end{aligned}
\end{equation} 
and the associated strong from is obtained as 
\begin{equation}
 \Divb{\Ce : \symb{ \nabla \bu - \Bchi} + \Cc : \skewb{ \nabla \bu - \Bchi}} + \bbf  = \bzero \,,
 \end{equation}
 with the following boundary conditions
 \begin{equation}
 \bu = \tilde{\bu} \quad \textrm{on} \quad \partial \Omega^u_\textrm{D}\,, \quad \bt^u = \{ \Ce : \symb{ \nabla \bu - \Bchi} + \Cc : \skewb{ \nabla \bu - \Bchi} \} \cdot \bn \quad \textrm{on} \quad  \partial \Omega^u_\textrm{N} \,, 
 \end{equation}
 with $\partial \Omega^u_\textrm{D} \cap \partial \Omega^u_\textrm{N} = \emptyset $ and  $\partial \Omega^u_\textrm{D} \cup \partial \Omega^u_\textrm{N} = \partial \Omega $. 
 
In a similar way, the variation of the potential with respect to the distortion field $\Bchi$ ends with the following form
\begin{equation}
\begin{aligned}
 \delta_{\Bchi} \Pi =  - \int_{\Omega} & \{\Ce : \symb{ \nabla \bu - \Bchi} + \Cc : \skewb{ \nabla \bu - \Bchi} - \Cmicro : \sym \Bchi + \bM \} :  \delta {\Bchi} \, \textrm{d} V \\ 
 & + \mu \, \Lc^2  (\IL : \Curl \Bchi) : \Curl \delta {\Bchi} \, \textrm{d} V -  \int_{ \partial \Omega^\chi_N} \bT^\chi : \delta \Bchi \, \textrm{d} A = 0\,, 
 \end{aligned}
\end{equation}
and by using integration by parts and the Stocks theory, the previous equation turns into
\begin{equation}
\begin{aligned}
 \delta_{\Bchi} \Pi = &  - \int_{\Omega}  \{\Ce : \symb{ \nabla \bu - \Bchi} + \Cc : \skewb{ \nabla \bu - \Bchi} - \Cmicro : \sym \Bchi   - \mu \, l_c^2 \, \textrm{Curl}[ \IL : \textrm{Curl} \Bchi ] \\ &  + \bM \} :  \delta {\Bchi} \, \textrm{d} V -  \int_{ \partial \Omega^\chi_N}  \{ \sum_{i=1}^3  \left( \bT^{\chi(i)} - \mu \, \Lc^2 (\IL : \Curl{\Bchi})^i  \times \bn \right) \cdot \delta {\Bchi}^i  \}  \;\; \textrm{d}A  \\ &-  \int_{ \partial \Omega^\chi_D}  \mu \, \Lc^2 \{ \sum_{i=1}^3  \left(  \delta {\Bchi}^i    \times \bn \right) \cdot  (\IL : \Curl{\Bchi})^i   \}  \;\; \textrm{d}A 
 = 0\,, 
\end{aligned} 
\end{equation}
and we obtain the following strong form 
 \begin{equation}
\Ce : \symb{ \nabla \bu - \Bchi} + \Cc : \skewb{ \nabla \bu - \Bchi} - \Cmicro : \sym \Bchi  - \mu \, \Lc^2 \, \textrm{Curl}[ \IL : \textrm{Curl} \Bchi ]  + \bM = \bzero \,, 
\end{equation}
with the following boundary conditions
 \begin{equation}
 \Bchi \times \bn = \tilde{\Bchi} \times \bn \quad \textrm{on} \quad \partial \Omega^\chi_\textrm{D}\,, \quad  \bT^{\chi} = \mu \, \Lc^2 (\IL : \Curl{\Bchi})  \times \bn  \quad \textrm{on} \quad  \partial \Omega^\chi_\textrm{N} \,, 
 \end{equation}
 with $\partial \Omega^\chi_\textrm{D} \cap \partial \Omega^\chi_\textrm{N} = \emptyset $ and  $\partial \Omega^\chi_\textrm{D} \cup \partial \Omega^\chi_\textrm{N} = \partial \Omega $. 
 
 
 The micro-distortion tensor $\Bchi$ can be written for the general three-dimensional case in the following form:
\eb
\Bchi =
 \left[ \begin{array}{ccc}
\chi_{11} & \chi_{12} & \chi_{13} \\
\chi_{21} & \chi_{22} & \chi_{23} \\
\chi_{31} & \chi_{32} & \chi_{33} \\
\end{array}\right] =  \left[ \begin{array}{c}
{\Bchi^{(1)}}^T \\
{\Bchi^{(2)}}^T \\
{\Bchi^{(3)}}^T \\
\end{array}\right], \quad \textrm{with} \quad  \Bchi^{(i)} = \left[ \begin{array}{c}
\chi_{i1} \\
\chi_{i2} \\
\chi_{i3} \\
\end{array} \right]
\ee
\begin{figure}[ht]
\center
	\unitlength=1mm
	\begin{picture}(200,55)
	\put(50,0){\def\svgwidth{6.5cm}{\small\input{figures/rec_chi.eps_tex}}}
	\end{picture}
	\caption{Tangential Components of the distortion field $\Bchi$ in the two-dimensional case.}
\label{Figure:T2T1L}
\end{figure} \\
The continuity requirements are: 
\eb \llbracket \bn \times \Bchi^{(i)} \rrbracket = \bzero \quad \textrm{for} \quad  i={1,2,3}
\ee 

which leads to for the two-dimensional case:  \\
\eb
\begin{aligned}
&\llbracket \chi_{12} \rrbracket = 0, \quad \textrm{and} \quad \llbracket \chi_{22} \rrbracket = 0, \quad \textrm{on} \quad \Gamma_1, \\
&\llbracket \chi_{11} \rrbracket = 0, \quad \textrm{and} \quad \llbracket \chi_{21} \rrbracket = 0, \quad \textrm{on} \quad \Gamma_2. 
\end{aligned} 
\ee
We need row-wise approximation of  $\Bchi$, i.e. $\Bchi^{(i)} \in \textrm{H}(\curl,\B) \quad \textrm{for} \quad i=1,2,3$  


Thus,  Curl of $\Bchi$ reads
\eb
\Curl \Bchi = \left[ \begin{array}{c}
(\Curl \Bchi^{(1)})^T \\
(\Curl \Bchi^{(2)})^T \\
(\Curl \Bchi^{(3)})^T \\
\end{array}\right] = \left[\begin{array}{c|c|c}
 \chi_{13,2} - \chi_{12,3}	& \chi_{11,3} - \chi_{13,1}  &  \chi_{12,1} - \chi_{11,2} \\
 \chi_{23,2} - \chi_{22,3}	& \chi_{21,3} - \chi_{23,1}  &  \chi_{22,1} - \chi_{21,2} \\
 \chi_{33,2} - \chi_{32,3}	& \chi_{31,3} - \chi_{33,1}  &  \chi_{32,1} - \chi_{31,2} 
\end{array}\right],
\label{eq:curlP}
\ee
which is reduced for the two-dimensional case to
\eb
\textrm{Curl} \Bchi = 
\left[\begin{array}{c|c|c}
0	&   0  &  \chi_{12,1} - \chi_{11,2} \\
0   &   0  &  \chi_{22,1} - \chi_{21,2} \\
0	&   0  &  0 
\end{array}\right]
\label{eq:curlP2D}
\ee 

%=========================================================================
\sect{\hspace{-5mm}.  Weak forms of the relaxed micromorphic model}
{\bf First weak form}: 
\begin{equation}
\delta \Pi_u = - \int_{\B}  \{ \Divb{\Ce : \symb{ \nabla \bu - \Bchi} + \Cc : \skewb{ \nabla \bu - \Bchi}} + \bbf \} \cdot \delta\bu \; \textrm{d}V  = 0
\end{equation}
turns to 
\begin{equation}
\begin{aligned}
\delta \Pi_u = \int_{\B}  - \Divb{ \delta\bu \cdot \Ce : \symb{ \nabla \bu - \Bchi}} + \nabla \delta\bu : \Ce : \symb{ \nabla \bu - \Bchi} &  \\  - \Divb{ \delta\bu \cdot \Cc : \skewb{ \nabla \bu - \Bchi}} + \nabla\delta\bu : \Cc : \skewb{ \nabla \bu - \Bchi} &  \\
\; -  \bbf \cdot \delta\Beta & \;\; \textrm{d}V  = 0\;,
\end{aligned}
\end{equation}
using the divergence theorem, we obtain
\begin{equation}
\label{eq:weakform1}
\begin{aligned}
\delta \Pi_u = \int_{\B} & \{\underbrace{\Ce : \symb{ \nabla \bu - \Bchi}}_{\Bsigma^\textrm{e}} + \underbrace{\Cc : \skewb{ \nabla \bu - \Bchi}}_{\Bsigma^\textrm{c}} \} : \nabla \delta\bu  - \bbf \cdot \delta\bu \;\; \textrm{d}V  \\
- \int_{\partial\B}  &\{ \underbrace{\left( \Ce : \symb{ \nabla \bu - \Bchi} + \Cc : \skewb{ \nabla \bu - \Bchi} \right) \cdot \bn}_{\bt^{u}}\}  \cdot \delta\bu  \;\; \textrm{d}A = 0\;,
\end{aligned}
\end{equation}
and the finial form reads 
\begin{equation}
\delta \Pi_u = \int_{\B}  \{ \Bsigma^\textrm{e}+ \Bsigma^\textrm{c} \} : \nabla\delta\bu  - \bbf \cdot \delta\bu \;\; \textrm{d}V  \\
- \int_{\partial\B}   \bt^{u} \cdot \delta\bu  \;\; \textrm{d}A = 0\;.
\end{equation}
{\bf Second weak form}: 
\begin{equation}
\begin{aligned}
\delta \Pi_\chi = \int_{\B}  & \{\Ce : \symb{ \nabla \bu - \Bchi} + \Cc : \skewb{ \nabla \bu - \Bchi} - \Cmicro : \sym \Bchi  \\ & - \mu \, l_c^2 \, \textrm{Curl}[ \IL : \textrm{Curl} \Bchi ] \} :  \delta {\Bchi} \; \textrm{d}V  = 0 \\ 
\end{aligned}
\end{equation}
which becomes 
\begin{equation}
\begin{aligned}
\delta \Pi_\chi = \int_{\B}  & \{\Ce : \symb{ \nabla \bu - \Bchi} + \Cc : \skewb{ \nabla \bu - \Bchi} - \Cmicro : \sym \Bchi  \} :  \delta {\Bchi}  \\  
& -  \mu \, l_c^2  (\IL : \Curl \Bchi) : \Curl \delta {\Bchi} - \mu \, l_c^2 \Divb{ \sum_{i=1}^3 \delta {\Bchi}^i \, \times \, (\IL :\Curl{\Bchi})^i } \;\; \textrm{d}V =  0
\end{aligned}
\end{equation} 
and the final form reads 
\begin{equation}
\label{eq:weakform2}
\begin{aligned}
\delta \Pi_\chi = \int_{\B}  & \{ \underbrace{\Ce : \symb{ \nabla \bu - \Bchi}}_{\Bsigma^\textrm{e}} + \underbrace{\Cc : \skewb{ \Grad \bu - \Bchi}}_{\Bsigma^\textrm{c}} - \Cmicro : \sym \Bchi  \} :  \delta {\Bchi}  \\  
&  -  \mu \, l_c^2 ( \IL : \Curl \Bchi) : \Curl \delta {\Bchi}  \;\; \textrm{d}V - \int_{\partial\B}  \mu \, l_c^2 \{ \sum_{i=1}^3 \delta {\Bchi}^i \, \times \, (\IL : \Curl{\Bchi})^i \}  \cdot \bn \;\; \textrm{d}A =  0
\end{aligned}
\end{equation} 
where $\delta {\Bchi}^i$ and $(\IL : \Curl{\Bchi})^i$ represent the rows of second order tensors $\delta {\Bchi}$ and $ \IL : \Curl{\Bchi}$.  
The last term can be rewritten in an alternative way as 
\begin{equation}
 \int_{\partial\B}  \mu \, l_c^2 \{ \sum_{i=1}^3 \delta {\Bchi}^i \, \times \, (\IL : \Curl{\Bchi})^i \}  \cdot \bn \;\; \textrm{d}A =   \int_{\partial\B}  \underbrace{\mu \, l_c^2 \{ \sum_{i=1}^3  \left( (\IL : \Curl{\Bchi})^i  \times \bn \right) \cdot \delta {\Bchi}^i  \}}_{\bT^\chi :  \delta {\Bchi}}  \;\; \textrm{d}A 
\end{equation}

%=========================================================================
\sect{\hspace{-5mm}. Approximation spaces}
\vspace{-4mm}
\ssect{\hspace{-5mm}. Lagrange elements}
\sssect{\hspace{-5mm}. T2T1 $H^1(\B) \times H^1(\B) $  element\\} We uses 6 nodes triangular element for the displacement field $\bu$ with quadratic shape functions. For the distortion field $\Bchi$, we use 3 nodes with linear shape functions, see Figure \ref{Figure:T2T1}. 
\begin{figure}[ht]
\center
\begin{tabular}{ l |l| l }
	\unitlength=1mm
	\begin{picture}(45,30)
	\put(0,-20){\def\svgwidth{4.5cm}{\small\input{figures/T2T1Lagrange.eps_tex}}}
	\end{picture} &
	\begin{tabular}{ c }
	 Displacement ansatz functions: \\
$ N^u_1 = (-1 + \eta + \xi) (-1 + 2 \eta + 2 \xi)$\\
$ N^u_2 = \xi (-1 + 2 \xi)$\\
$ N^u_3 = \eta (-1 + 2 \eta)$\\
$ N^u_4 = -4 \xi (-1 + \eta + \xi)$\\
$ N^u_5 = 4 \eta \xi$\\
$ N^u_6 =-4 \eta (-1 + \eta + \xi)$\\
\\
\\
		\end{tabular} 
	  &  	
	  \begin{tabular}{ c }
	$\Bchi$ ansatz functions: \\
$ N^\chi_1 = 1- \eta - \xi$\\
$ N^\chi_2 = \xi$\\
$ N^\chi_3 = \eta$\\  
 \\
 \\ 
 \\
 \\
 \\
		\end{tabular} 
	\end{tabular} 
	\caption{T2T1 element topology. Nodes with displacement degree of freedoms are shown as filled circles and nodes used for the distortion field $\Bchi$ appear as hollow squares.}
\label{Figure:T2T1}
\end{figure} 


Geometry and displacement field approximation\\
\begin{equation}
 \bX(\Bxi) = \sum_{I=1}^6 N^u_I(\Bxi)  \bX_I\,, \qquad \bu(\Bxi) = \sum_{I=1}^6 N^u_I(\Bxi)  \bd^u_I\,. 
\end{equation}
Deformation gradient approximation: 
\begin{equation}
\nabla \bu = \sum_{I=1}^6 \bd^u_I \otimes \nabla N^u_I(\Bxi)\,, \quad \textrm{with} \quad 
\nabla {N^u_I(\Bxi)} = \bJ^{-T} \cdot \nabla_\Bxi N^u_{I}\,,
\end{equation}
where $\bJ$ is Jacobian. The distortion field $\Bchi$ is interpolated as  
\begin{equation}
\Bchi =   \sum_{I=1}^{3}   N^\chi_I(\Bxi)  \bD^\chi_I
\end{equation}
where  $\bD^\chi_I$ is the second order tensorial  degree of freedom of node $I$. \\
The distortion field $\Bchi$ will be treated as row vectors to calculate its rotation, so we have for the two-dimensional case 
\begin{equation}
\Bchi 
= \left[\begin{array}{c c}
\chi_{11}  \quad \chi_{12} \\ 
\chi_{21} \quad  \chi_{22}
\end{array}\right]  = \left[\begin{array}{c c}
{\Bchi^{(1)}}^T \\ 
{\Bchi^{(2)}}^T
\end{array}\right]
= \sum_{I=1}^{3}  N^\chi_I(\Bxi) \left[\begin{array}{c c}
{D^\chi_{11}}_I  \quad {D^\chi_{12}}_I \\ 
{D^\chi_{21}}_I \quad  {D^\chi_{22}}_I 
\end{array}\right] 
,
\end{equation}
and the gradient field of the previous vectors read
\begin{equation}
\nabla \Bchi^{(I)} = \bJ^{-T} \cdot \nabla_\Bxi \Bchi^{(I)}\,,
\end{equation}
and the rotation of the vector $\Bchi_i$ reads 
\begin{equation}
\Curl^{2D}{\Bchi^{(I)}} = \nabla \Bchi^{(I)}_{21} - \nabla \Bchi^{(I)}_{12}\,,
\end{equation}
where $\Curl^{2D}{\Bchi^{(1)}}=  \Curl{\Bchi}_{13}$ and $\Curl^{2D}{\Bchi^{(2)}} =  \Curl{\Bchi}_{23}$. 
\newpage


\ssect{\hspace{-5mm}. $ H(\curl, \B)$ elements}
\sssect{\hspace{-5mm}. Q2NQ1 $H^1(\B) \times H(\curl, \B)$ element\\} 
The displacement field $\bu$ is discretized using Lagrange ansatz function with 9 nodes while the distortion field $\Bchi$  is discretized using a distortion vector $\bd^\chi_I$ defined on the center of the four edges  with vectorial  ansatz functions of $H(\curl)$ type. 
The parametric element is shown in Figure \ref{Figure:Q2NQ1} with $\xi \in [-1,1]$ and $\eta \in [-1,1]$.


\begin{figure}[ht]
\center
\begin{tabular}{ l |l| l }
	\unitlength=1mm
	\begin{picture}(45,30)
	\put(0,-20){\def\svgwidth{4.5cm}{\small\input{figures/Q2Q1.eps_tex}}}
	\end{picture} &
	\begin{tabular}{ c }
	 Displacement ansatz functions: \\
$ N^u_1 = ( \xi^2 - \xi )(\eta^2 - \eta)/4\,$ \\
$ N^u_2 = (\xi^2 + \xi )(\eta^2 - \eta)/4\,$ \\
$ N^u_3 = (\xi^2 + \xi )(\eta^2 + \eta)/4\,$ \\
$ N^u_4 = (\xi^2 - \xi )(\eta^2 + \eta)/4\,$ \\
$ N^u_5 = (\eta^2 - \eta)(1 - \xi^2 )/2\,$ \\ 
$ N^u_6 = (\xi^2 + \xi )(1 - \eta^2 )/2\,$ \\ 
$ N^u_7 = (\eta^2 + \eta)(1 - \xi^2 )/2\,$ \\
$ N^u_8 = (\xi^2 - \xi )(1 - \eta^2 )/2\,$ \\
$ N^u_9 = (1 - \xi^2 )(1 - \eta^2 )\,$

		\end{tabular} 
	  &  	
	  \begin{tabular}{ c }
	$\Bchi$ vectorial  ansatz functions: \\
$\bv^\chi_{1} =  \left( \begin{array}{c}
(-\eta + 1)/2  \\
0 
\end{array} \right)$ \\ 

$\bv^\chi_{2} =  \left( \begin{array}{c}
0 \\
 (\xi + 1)/2 
\end{array} \right)$ \\

$\bv^\chi_{3} =  \left( \begin{array}{c}
(\eta + 1)/2 \\
0
\end{array} \right)$\\

$\bv^\chi_{4} =  \left( \begin{array}{c}
0 \\
 (-\xi + 1)/2 
\end{array}\right)$.\\

		\end{tabular} 
	\end{tabular} 
	\caption{Q2NQ1 element topology. Nodes with displacement degree of freedoms are shown as filled circles and red arrows demonstrate edges used for the distortion field discretization.}
\label{Figure:Q2NQ1}
\end{figure} 

{\bf Discretization:} 

Geometry and displacement field approximation\\
\begin{equation}
 \bX(\Bxi) = \sum_{I=1}^9 N^u_I(\Bxi)  \bX_I\,, \qquad \bu(\Bxi) = \sum_{I=1}^9 N^u_I(\Bxi)  \bd^u_I\,. 
\end{equation}
Deformation gradient approximation: 
\begin{equation}
\nabla \bu = \sum_{I=1}^9 \bd^u_I \otimes \nabla_\bX N^u_I(\Bxi)\,, \quad \textrm{with} \quad 
\nabla_\bX {N^u_I(\Bxi)} = \bJ^{-T} \cdot \nabla_\Bxi N^u_{I}.
\end{equation}
 The vectorial  ansatz functions are mapped from the parametric space to the physical space (reference configuration) by the so-called the covariant Piola transformation. Furthermore, we multiply with the associated  edge length ${l_e}_I$ and divide by two (edge length of the parameter element) to enforce a constant value of one on the related edge and not any another constant value. Furthermore, we multiply with $\alpha_I$ to quarantine the global consistency of the tangential components of the mapped vectors on the neighboring edges
\begin{equation}
\Bpsi^\chi_I = \frac{{\alpha_I l_e}_I}{2} \bJ^{-T} \cdot \bv^\chi_I\,.
\end{equation}
The distortion field $\Bchi$ is interpolated as (Appendix A.3)
\begin{equation}
\Bchi =   \sum_{I=1}^{4}  \bd^\chi_I \otimes \Bpsi^\chi_I\,.
\end{equation}
The rotation of the the distortion field is obtained then by 
\begin{equation}
 \Curl_\bX{\Bchi} =   \sum_{i=1}^{4}  \bd^\chi_I \otimes  \Curl_\bX{\Bpsi^\chi_I}\,, 
\end{equation}
 with 
\begin{equation}
\Curl_\bX{\Bpsi^\chi_I} = \frac{{\alpha_I l_e}_I}{2 \det{\bJ}} \bJ \cdot \Curl_{\Bxi}\bv^\chi_I\,,
\end{equation}
which is reduced to the following for the 2D case 
\begin{equation}
\Curl^{2D}_\bX{\Bpsi_I} = \frac{{\alpha_I l_e}_I}{2 \det{\bJ}} \Curl^{2D}_{\Bxi}\bv^\chi_I\,,
\end{equation}
where $\Curl^{2D}_{\Bxi}\bv^\chi_{I =1,2} = -  \Curl^{2D}_{\Bxi}\bv^\chi_{I =3,4}  = \frac{1}{2}\,.$  
\sssect{\hspace{-5mm}. Q2NQ2 $H^1(\B) \times H(\curl, \B)$ element\\} 
We use the standard second-order formulation for displacement field with Lagrange basis functions similar to Q2NQ1 and we use second-order N\'ed\'elec vectorial shape functions with vectorial degree of freedoms defined in 8 nodes at element edges and 4 inner nodes. The second-order N\'ed\'elec basis functions for quadrilateral element read
\begin{equation}
\bv^\chi =  \left( \begin{array}{c}
a_1 + a_2 \xi + a_3 \eta + a_4 \xi*\eta + a_5 \eta^2 + 
 a_6 \xi \eta^2 \\ a_7 + a8 \xi + a_9 \eta + 
 a_{10} \xi*\eta + a_{11} \xi^2 + a_{12} \eta \xi^2
\end{array} \right) \,.
\end{equation}
A system of equations needs to be constructed to obtain the N\'ed\'elec basis functions by calculating the inner and outer degree of freedoms (moments). The edge degree of freedoms are defined as 
\begin{equation}
m_{ij} = \int_{e_i} (\bv^\chi \cdot \bt_i)  \, q_{j} \, ds \,, \quad \forall q_j \in \IP_{k-1}(e_i)\,
\end{equation}
and for inner degree of freedoms, they read 
\begin{equation}
m_{i} = \int_{\B} \bv^\chi \cdot \bq_{i} \, ds \,, \quad \forall  \bq_i \in Q_{k-1,k-2} \times Q_{k-2,k-1}\,
\end{equation}
\begin{center}
\begin{table}[ht]
\begin{tabular}{|c|c|c|c|c|}
\cline{1-5}
$i$ &  $q_j/\bq_i$ & $t_i$ &  $\xi-\eta$ coloration & $m_{ij}/m_i$   \\  \cline{1-5}
1 & $1/2 - 3/4 \, \xi$ & $(1,0)^T$ & $\eta = -1$ & $1/2(2a_1 - a_2 - 2a_3 + a_4 + 2a_5 - a_6)$ \\
\cline{1-5}
2 & $1/2 + 3/4 \, \xi$ & $(1,0)^T$ & $\eta = -1$ & $1/2(2a_1 + a_2 - 2a_3 - a_4 + 2a_5 + a_6)$ \\
\cline{1-5}
3 & $1/2 - 3/4 \, \eta$ & $(0,1)^T$ & $\xi = 1$ & $1/2(-a_{10} + 2a_{11} - a_{12} + 2a_7 + 2a_8 - a_9)$ \\
\cline{1-5}
4 & $1/2 + 3/4 \, \eta$ & $(0,1)^T$ & $\xi = 1$ & $1/2(a_{10} + 2a_{11} + a_{12} + 2a_7 + 2a_8 + a_9)$ \\
\cline{1-5}
5 & $1/2 + 3/4 \, \xi$ & $(1,0)^T$ & $\eta = 1$ & $1/2(2a_1 + a_2 + 2a_3 + a_4 + 2a_5 + a_6)$ \\
\cline{1-5}
6 & $1/2 - 3/4 \, \xi$ & $(1,0)^T$ & $\eta = 1$ & $1/2(2a_1 - a_2 + 2a_3 - a_4 + 2a_5 - a_6)$ \\
\cline{1-5}
7 & $1/2 + 3/4 \, \eta$ & $(0,1)^T$ & $\xi = -1$ & $1/2(-a_{10} + 2a_{11} + a_{12} + 2a_{7} - 2a_{8} + a_9)$ \\
\cline{1-5}
8 & $1/2 - 3/4 \, \eta$ & $(0,1)^T$ & $\xi = -1$ & $1/2(a_{10} + 2a_{11} - a_{12} + 2a_7 - 2a_8 - a_9)$ \\
\cline{1-5}
9 &  $(3/8 + 9/16 \xi,0)^T$& - & -& $1/4 (6 a_1 + 3 a_2 + 2 a_5 + a_6)$ \\
\cline{1-5}
10 &  $(3/8 - 9/16 \xi,0)^T$& - & -& $1/4 (6 a_1 - 3 a_2 + 2 a_5 - a_6)$ \\
\cline{1-5}
11 &  $(0,3/8 + 9/16 \eta)^T$& - & -& $1/4 (2 a_{11} + a_{12} + 6 a_7 + 3 a_9)$ \\
\cline{1-5}
12 &  $(0,3/8 - 9/16 \eta)^T$& - & -& $1/4 (2 a_{11} - a_{12} + 6 a_7  - 3 a_9)$ \\
\cline{1-5}
\end{tabular}
\end{table}
\end{center}
The N\'ed\'elec  basis functions ($\bv_i^\chi$) are obtained by enforcing a value of one for a single moment and zeros for the rest: 
\begin{equation}
\begin{aligned}
\bv_1^\chi &= \left( \begin{array}{c} 
-1/8 - \eta/4 + 3 \eta^2/8 + \xi/4 + \eta \xi/2 - 
 3 \eta^2 \xi/4 \\
0
 \end{array} \right), \\
  \bv_2^\chi &= \left( \begin{array}{c} 
 -1/8 - \eta/4 + 3 \eta^2/8 - \xi/4 - \eta \xi/2 + 
 3 \eta^2 \xi/4 \\
0
 \end{array} \right), \\
  \bv_3^\chi & = \left( \begin{array}{c} 
0 \\
-1/8 + \eta/4 + \xi/4 - \eta\xi/2 + 3\xi^2/8 - 3\eta \xi^2/4
 \end{array} \right), \\
 \bv_4^\chi &= \left( \begin{array}{c} 
0 \\
-1/8 - \eta/4 + \xi/4 + \eta\xi/2 + 3\xi^2/8 +  3\eta\xi^2/4 
 \end{array} \right), \\
  \bv_5^\chi &= \left( \begin{array}{c} 
-1/8 + \eta/4 + 3\eta^2/8 - \xi/4 + \eta \xi]/2 +  3 \eta^2\xi/4 \\
0
 \end{array} \right), \\
 \bv_6^\chi &= \left( \begin{array}{c} 
-1/8 + \eta/4 + 3\eta^2/8 + \xi/4 - \eta\xi/2 -  3\eta^2\xi)/4 \\
0
 \end{array} \right), \\
  \bv_7^\chi &= \left( \begin{array}{c} 
0 \\
-1/8 - \eta/4 - \xi/4 - \eta\xi/2 + 3\xi^2/8 +  3 \eta\xi^2/4
 \end{array} \right), \\
  \bv_8^\chi &= \left( \begin{array}{c} 
0 \\
-1/8 + \eta/4 - \xi/4 + \eta \xi/2 + 3\xi^2/8 -  3\eta\xi^2/4
 \end{array} \right)\,.
  \\
  \bv_9^\chi &= \left( \begin{array}{c} 
1/2 - \eta^2/2 + \xi - \eta^2 \xi \\
0
 \end{array} \right)\,, \quad  \bv_{10}^\chi = \left( \begin{array}{c} 
1/2 - \eta^2/2 - \xi + \eta^2 \xi \\
0
 \end{array} \right)\,, \\
   \bv_{11}^\chi &= \left( \begin{array}{c} 
0 \\
1/2 + \eta - \xi^2/2 - \eta \xi^2
 \end{array} \right)\,, \quad  \bv_{12}^\chi = \left( \begin{array}{c} 
0 \\
1/2 - \eta - \xi^2/2 + \eta \xi^2
 \end{array} \right)\,.
 \end{aligned}
\end{equation}
\begin{figure}[ht]
\center
	\unitlength=1mm
	\begin{picture}(85,70)
	\put(0,0){\def\svgwidth{8cm}{\small\input{figures/Q2Q2.eps_tex}}}
	\end{picture}
	\caption{Q2NQ2 element topology. Nodes with displacement degree of freedoms are shown as filled circles and red x demonstrate nodes used for the distortion field discretization with vectorial degree of freedoms.}
\label{Figure:Q2NQ2}
\end{figure} 

{\bf Discretization:} 

Geometry and displacement field approximation\\
\begin{equation}
 \bX(\Bxi) = \sum_{I=1}^9 N^u_I(\Bxi)  \bX_I\,, \qquad \bu(\Bxi) = \sum_{I=1}^6 N^u_I(\Bxi)  \bd^u_I\,. 
\end{equation}
Deformation gradient approximation: 
\begin{equation}
\nabla \bu = \sum_{I=1}^9 \bd^u_I \otimes \nabla_\bX N^u_I(\Bxi)\,, \quad \textrm{with} \quad 
\nabla_\bX {N^u_I(\Bxi)} = \bJ^{-T}  \cdot \nabla_\Bxi N^u_{I}\,.
\end{equation}
The vectorial  basis functions are mapped from the parametric space to the physical space (reference configuration) by so-called the covariant Piola transformation. Furthermore, we multiply with the associated edge length divided by two (${l_e}_I/2$) to enforce a constant value of one on the related edge and not any another constant value. Furthermore, we multiply with $\alpha_I$ to quarantine the global consistency of the tangential components of the mapped vectors on the neighboring edges
\begin{equation}
\Bpsi^\chi_I = \alpha_I \frac{{l_e}_I}{2} \bJ^{-T} \cdot \bv^\chi_I\,.
\end{equation}
The distortion field $\Bchi$ is interpolated as  (Appendix A.3)
\begin{equation}
\Bchi =   \sum_{I=1}^{12}   \bd^\chi_I \otimes \Bpsi^\chi_I \,. 
\end{equation}
The rotation of the the distortion field is obtained then by 
\begin{equation}
\Curl_\bX{\Bchi} =   \sum_{I=1}^{12}   \bd^\chi_I \otimes \Curl_\bX{\Bpsi^\chi_I}\,, 
\end{equation}
 with 
\begin{equation}
\Curl_\bX{\Bpsi^\chi_I} = \frac{{\alpha_I l_e}_I}{2\det{\bJ}} \bJ \cdot \Curl_{\Bxi}\bv^\chi_I\,,
\end{equation}
which is reduced to the following for the 2D case 
\begin{equation}
\Curl^{2D}_\bX{\Bpsi^\chi_I} =  \frac{{\alpha_I l_e}_I}{2\det{\bJ}}  \Curl^{2D}_{\Bxi}\bv^\chi_I\,.
\end{equation}

\FloatBarrier
\sssect{\hspace{-5mm}. T2NT1 $H^1(\B) \times H(\curl,\B)$ element\\} 
Displacement field $\bu$ is discretized using Lagrange ansatz functions with 6 nodes.  A vectorial degree of freedom $\bd^\chi_I$ on the center of each edge are used for discretizing $\Bchi$ with tangential conforming shape functions. The parameter element is described in Figure  \ref{Figure:T2NT1} with  $\xi,\eta \in [-1,1]$.

\begin{figure}[ht]
\center
\begin{tabular}{ l |l| l }
	\unitlength=1mm
	\begin{picture}(45,30)
	\put(0,-20){\def\svgwidth{4.5cm}{\small\input{figures/T2T1.eps_tex}}}
	\end{picture} &
	\begin{tabular}{ c }
	 Displacement ansatz functions: \\
$ N^u_1 = (-1 + \eta + \xi) (-1 + 2 \eta + 2 \xi)$\\
$ N^u_2 = \xi (-1 + 2 \xi)$\\
$ N^u_3 = \eta (-1 + 2 \eta)$\\
$ N^u_4 = -4 \xi (-1 + \eta + \xi)$\\
$ N^u_5 = 4 \eta \xi$\\
$ N^u_6 =-4 \eta (-1 + \eta + \xi)$\\
\\
\\
		\end{tabular} 
	  &  	
	  \begin{tabular}{ c }
	$\Bchi$ vectorial ansatz functions: \\
$\bv^\chi_1 =  \left( \begin{array}{c}
1 - \eta \\ 
\xi
\end{array} \right)$ \\ 
$\bv^\chi_2 =  \left( \begin{array}{c}
\eta \\ 
- \xi
\end{array} \right)$ \\
$\bv^\chi_3 =  \left( \begin{array}{c}
\eta \\
 1 - \xi
\end{array} \right)$ \\
\\
\\
		\end{tabular} 
	\end{tabular} 
	\caption{T2NT1 element topology. Nodes with displacement degree of freedoms are shown as filled circles and red arrows demonstrate edges used for the distortion field discretization.}
\label{Figure:T2NT1}
\end{figure} 

{\bf Discretization:} 

Geometry and displacement field approximation\\
\begin{equation}
 \bX(\Bxi) = \sum_{I=1}^6 N^u_I(\Bxi)  \bX_I\,, \qquad \bu(\Bxi) = \sum_{I=1}^6 N^u_I(\Bxi)  \bd^u_I\,. 
\end{equation}
Deformation gradient approximation: 
\begin{equation}
\nabla \bu = \sum_{I=1}^6 \bd^u_I \otimes \nabla_\bX N^u_I(\Bxi)\,, \quad \textrm{with} \quad 
\nabla_\bX {N^u_I(\Bxi)} = \bJ^{-T}  \cdot \nabla_\Bxi N^u_{I}\,.
\end{equation}
The vectorial  ansatz functions are mapped from the parametric space to the physical space (reference configuration) by so-called the covariant Piola transformation. Furthermore, we multiply with the associated edge length ${l_e}_I$ to enforce a constant value of one on the related edge and not any another constant value. Furthermore, we multiply with $\alpha_I$ to quarantine the global consistency of the tangential components of the mapped vectors on the neighboring edges
\begin{equation}
\Bpsi^\chi_I = {\alpha_I l_e}_I \bJ^{-T} \cdot \bv^\chi_I\,.
\end{equation}
The distortion field $\Bchi$ is interpolated as  (Appendix A.3)
\begin{equation}
\Bchi =   \sum_{I=1}^{3}   \bd^\chi_I \otimes \Bpsi^\chi_I \,. 
\end{equation}
The rotation of the the distortion field is obtained then by 
\begin{equation}
\Curl_\bX{\Bchi} =   \sum_{I=1}^{3}   \bd^\chi_I \otimes \Curl_\bX{\Bpsi^\chi_I}\,, 
\end{equation}
 with 
\begin{equation}
\Curl_\bX{\Bpsi^\chi_I} = \frac{{\alpha_I l_e}_I}{\det{\bJ}} \bJ \cdot \Curl_{\Bxi}\bv^\chi_I\,,
\end{equation}
which is reduced to the following for the 2D case 
\begin{equation}
\Curl^{2D}_\bX{\Bpsi^\chi_I} =  \frac{{\alpha_I l_e}_I}{\det{\bJ}}  \Curl^{2D}_{\Bxi}\bv^\chi_I\,,
\end{equation}
where $\Curl^{2D}_{\Bxi}\bv^\chi_{I =1}=2$ and  $\Curl^{2D}_{\Bxi}\bv^\chi_{I=2,3}=-2$ . 


\sssect{\hspace{-5mm}. T2NT2 $H^1(\B) \times H(\curl,\B)$ element\\} 
We use second-order formulation for both fields. Displacement field $\bu$ is discretized using Lagrange ansatz functions with 6 nodes.  The micro-distortion field is defined on eight nodes with vectorial degree of freedom (six on edges and two internal ones). Second-order N\'ed\'elec triangular element is based on the following polynomial (see A.6.1)
\begin{equation}
\bv^\chi =  \left( \begin{array}{c}
a_1 + a_2 \xi + a_3 \eta - a_7 \eta^2 - a_8 \xi\eta \\
a_4 + a_5 \xi + a_6 \eta + a_7 \eta\xi + a_8 \xi^2
\end{array} \right) \,.
\end{equation}
A system of equations needs to be constructed to obtain the N\'ed\'elec basis functions by calculating the inner and outer degree of freedoms (moments). The edge degree of freedoms are defined as 
\begin{equation}
m_{ij} = \int_{e_i} (\bv^\chi \cdot \bt_i)  \, q_{j} \, ds \,, \quad \forall q_j \in \IP_{k-1}(e_i)\,
\end{equation}
and for inner degree of freedoms, they read 
\begin{equation}
m_{i} = \int_{\B} \bv^\chi \cdot \bq_{i} \, ds \,, \quad \forall \bq_i \in (\IP_{k-2})^2\,
\end{equation}
\begin{center}
\begin{table}[ht]
\begin{tabular}{|c|c|c|c|c|}
\cline{1-5}
$i$ &  $q_j/\bq_i$ & $t_i$ &  $\xi-\eta$ coloration & $m_{ij}/m_i$   \\  \cline{1-5}
1 & $2 \xi$ & $(\frac{1}{\sqrt{2}},-\frac{1}{\sqrt{2}})^T$ & $\eta = 1 - \xi$ & $1/3 (3 a_1 + 2 a_2 + a_3 - 3 a_4 - 2 a_5 - a_6 - a_7 - 2 a_8)$ \\
\cline{1-5}
2 & $2 \eta$ & $(\frac{1}{\sqrt{2}},-\frac{1}{\sqrt{2}})^T$ & $\xi = 1 - \eta$ & $1/3 (3 a_1 + a_2 + 2 a_3 - 3 a_4 - a_5 - 2 a_6 - 2 a_7 - a_8)$\\
\cline{1-5}
3 & $2 \eta$ & $(0,1)^T$ & $\xi = 0$ & $a_4 + 2 a_6/3$ \\
\cline{1-5}
4& $2 (1 - \eta)$ & $(0,1)^T$ & $\xi = 0$ & $a_4 + a_6/3$ \\
\cline{1-5}
5& $2 (1 - \xi)$ & $(1,0)^T$ & $\eta = 0$ & $a_1 + a_2/3$  \\
\cline{1-5}
6& $2\xi$ & $(1,0)^T$ & $\eta = 0$ & $a_1 + 2 a_2/3$ \\
\cline{1-5}
7& $(0,2)^T$ &-& - & $1/12 (12 a_4 + 4 a_5 + 4 a_6 + a_7 + 2 a_8)$ \\
\cline{1-5}
8& $(2,0)^T$ &-& - & $1/12 (12 a_1 + 4 a_2 + 4 a_3 - 2 a_7 - a_8)$  \\
\cline{1-5}
\end{tabular}
\end{table}
\end{center}
The N\'ed\'elec  basis functions ($\bv_i^\chi$) are obtained by enforcing a value of one for a single moment and zeros for the rest: 
\begin{equation}
\begin{aligned}
\bv_1^\chi &= \left( \begin{array}{c} 
-\eta + 4 \eta \xi \\
 2 \xi - 4 \xi^2 
 \end{array} \right),  \bv_2^\chi = \left( \begin{array}{c} 
-2 \eta + 4 \eta^2 \\
\xi - 4 \eta \xi
 \end{array} \right),  \bv_3^\chi = \left( \begin{array}{c} 
-2 \eta + 4 \eta^2 \\
 -1 + 3 \eta + \xi - 4 \eta \xi
 \end{array} \right), \\
 \bv_4^\chi &= \left( \begin{array}{c} 
3 \eta - 4 \eta^2 - 4 \eta \xi \\
 2 - 3 \eta - 6 \xi + 4 \eta \xi + 4 \xi^2
 \end{array} \right),  \bv_5^\chi = \left( \begin{array}{c} 
2 - 6 \eta + 4 \eta^2 - 3 \xi + 4 \eta \xi \\
 3 \xi - 4 \eta \xi - 4 \xi^2
 \end{array} \right), \\
 \bv_6^\chi &= \left( \begin{array}{c} 
-1 + \eta + 3 \xi - 4 \eta \xi \\
 -2 \xi + 4 \xi^2
 \end{array} \right), 
  \bv_7^\chi = \left( \begin{array}{c} 
-4 \eta + 4 \eta^2 + 8 \eta \xi \\
8 \xi - 4 \eta \xi - 8 \xi^2
 \end{array} \right), \\
  \bv_8^\chi &= \left( \begin{array}{c} 
8 \eta - 8 \eta^2 - 4 \eta \xi \\
-4 \xi + 8 \eta \xi +  4 \xi^2
 \end{array} \right)\,.
 \end{aligned}
\end{equation}
\begin{figure}[ht]
\center
	\unitlength=1mm
	\begin{picture}(45,55)
	\put(0,0){\def\svgwidth{5.5cm}{\small\input{figures/T2T2.eps_tex}}}
	\end{picture}
	\caption{T2NT2 element topology. Nodes with displacement degree of freedoms are shown as filled circles and red x demonstrate nodes used for the distortion field discretization with vectorial degree of freedoms.}
\label{Figure:T2NT2}
\end{figure} 

{\bf Discretization:} 

Geometry and displacement field approximation\\
\begin{equation}
 \bX(\Bxi) = \sum_{I=1}^6 N^u_I(\Bxi)  \bX_I\,, \qquad \bu(\Bxi) = \sum_{I=1}^6 N^u_I(\Bxi)  \bd^u_I\,. 
\end{equation}
Deformation gradient approximation: 
\begin{equation}
\nabla \bu = \sum_{I=1}^6 \bd^u_I \otimes \nabla_\bX N^u_I(\Bxi)\,, \quad \textrm{with} \quad 
\nabla_\bX {N^u_I(\Bxi)} = \bJ^{-T}  \cdot \nabla_\Bxi N^u_{I}\,.
\end{equation}
The vectorial  basis functions are mapped from the parametric space to the physical space (reference configuration) by so-called the covariant Piola transformation. Furthermore, we multiply with the associated edge length ${l_e}_I$ to enforce a constant value of one on the related edge and not any another constant value. Furthermore, we multiply with $\alpha_I$ to quarantine the global consistency of the tangential components of the mapped vectors on the neighboring edges
\begin{equation}
\Bpsi^\chi_I = {\alpha_I l_e}_I \bJ^{-T} \cdot \bv^\chi_I\,.
\end{equation}
The distortion field $\Bchi$ is interpolated as  (Appendix A.3)
\begin{equation}
\Bchi =   \sum_{I=1}^{8}   \bd^\chi_I \otimes \Bpsi^\chi_I \,. 
\end{equation}
The rotation of the the distortion field is obtained then by 
\begin{equation}
\Curl_\bX{\Bchi} =   \sum_{I=1}^{8}   \bd^\chi_I \otimes \Curl_\bX{\Bpsi^\chi_I}\,, 
\end{equation}
 with 
\begin{equation}
\Curl_\bX{\Bpsi^\chi_I} = \frac{{\alpha_I l_e}_I}{\det{\bJ}} \bJ \cdot \Curl_{\Bxi}\bv^\chi_I\,,
\end{equation}
which is reduced to the following for the 2D case 
\begin{equation}
\Curl^{2D}_\bX{\Bpsi^\chi_I} =  \frac{{\alpha_I l_e}_I}{\det{\bJ}}  \Curl^{2D}_{\Bxi}\bv^\chi_I\,.
\end{equation}
\sect{\hspace{-5mm}. Linearization and stiffness matrices}
We assume for this section that $\Cc=\bzero$ and $ \IL : \textrm{Curl} \Bchi = \textrm{Curl} \Bchi  $. The nonlinear system of equations is solved by the iterative Newton-Raphson scheme that requires the linearization of the weak forms of equilibrium.
 The linearization of  $\delta \Pi_u$  and $\delta \Pi_\chi$ in Equations (\ref{eq:weakform1}) and  (\ref{eq:weakform2}) gives  
\begin{equation}
\textrm{Lin} \delta \Pi_u = \delta \Pi_u + \Delta \delta \Pi_u, \quad \textrm{Lin} \delta \Pi_\chi = \delta \Pi_\chi + \Delta \delta \Pi_\chi. 
\end{equation}
The linearized form of the stress $\Bsigma^{e}$ reads 
\begin{equation}
\Delta \Bsigma^{e} = \Ce : \textrm{sym}(\nabla \Delta \bu) -  \Ce : \textrm{sym}( \Delta \Bchi),
\end{equation}
which leads to 
\begin{equation}
\Delta \delta \Pi_u = \int_{\B} \Delta \Bsigma^\textrm{e}: \nabla\delta\bu \; \textrm{d}V = \int_{\B} \textrm{sym}(\nabla\delta\bu) : \{ \Ce : \textrm{sym}(\nabla \Delta \bu) -  \Ce : \textrm{sym}( \Delta \Bchi) \} \; \textrm{d}V \,,
\end{equation}
and 
\begin{equation}
\delta \Pi_\chi = \int_{\B}  \{ \Delta \Bsigma^\textrm{e}  - \Cmicro : \sym \Delta \Bchi  \} :  \delta {\Bchi}    -  \mu \, l_c^2 \Curl  \Delta \Bchi : \Curl \delta {\Bchi}  \;\; \textrm{d}V  =  0
\end{equation}
which can be reformulated as 
\begin{equation}
\begin{aligned}
\delta \Pi_\chi = \int_{\B}  & \textrm{sym}\delta {\Bchi} : \{ - \Ce : \textrm{sym}(\nabla \Delta \bu) + \Ce : \textrm{sym}( \Delta \Bchi)  + \Cmicro : \sym \Delta \Bchi  \}  \\ & +  \mu \, l_c^2 \Curl  \delta \Bchi : \Curl \Delta {\Bchi}  \;\; \textrm{d}V  =  0
\end{aligned}
\end{equation}
 The continuum body is discretizated to $n^\textrm{ele}$ elements 
 \begin{equation}
 \B_0 \approx \B^h = \overset{n^\textrm{ele}}{\underset{e}{\bigcup}} \, \B^e\,.
 \end{equation}
 We define the following quantities in Voigt notation used to build up the element stiffness matrix. 
  The displacements is approximated as
 \begin{equation}
\bu = \sum_{I=1}^{n_u} \bN^u_I  \cdot \bd^u_I
\end{equation}
with
\begin{equation}
\bN^u_I =
\left(\begin{matrix}
N^u_{I}  & 0  \\
0 & N^u_{I} 
\end{matrix}\right)\,, \quad  \bd^u_I =
\left(\begin{matrix}
d^{u}_{(1)I} \\
d^{u}_{(2)I}
\end{matrix}\right)\,.
\end{equation}
 The symmetric gradient of the displacement is defined as 
\begin{equation}
\textrm{sym} \nabla \tilde{\bu} = \sum_{I=1}^{n_u} \bB^{u}_I \cdot  \bd^u_I
\end{equation} 
with 
\begin{equation}
\bB^{u}_I =
\left(\begin{matrix}
N^u_{I,1}  & 0 \\
0 & N^u_{I,2} \\
N^u_{I,2} & N^u_{I,1} \\
\end{matrix}\right), \quad \textrm{sym} \nabla \tilde{\bu} = 
\left(\begin{matrix}
u_{1,1} \\
u_{2,2} \\
u_{1,2} + u_{2,1}  \\
\end{matrix}\right)
\end{equation}
The symmetric part of the distortion field reads (Lagrange formulation)
\begin{equation}
\sym \tilde{\Bchi} =   \sum_{I=1}^{n_{\chi}}   \bN^\chi_I \cdot  \bD^\chi_I
\end{equation}
with 
\begin{equation}
 \bN^\chi_I =
\left(\begin{matrix}
N^\chi_{I}  & 0 & 0 & 0 \\
0 & N^\chi_{I}  & 0 & 0 \\
0 & 0 & N^\chi_{I} & N^\chi_{I} \\
\end{matrix}\right), \quad \textrm{sym}  \tilde{\Bchi} = 
\left(\begin{matrix}
\chi_{11} \\
\chi_{22} \\
\chi_{12} + \chi_{21}  \\
\end{matrix}\right),
\quad \bD^\chi_I = 
\left(\begin{matrix}
 D^\chi_{(11)I} \\
 D^\chi_{(22)I} \\
 D^\chi_{(12)I} \\
 D^\chi_{(21)I} \\ 
 \end{matrix}\right)\,.
\end{equation}
The curl operator of the micro-distortion field is defined for the two dimensional case as
\begin{equation}
\Curl \tilde{\Bchi} =  \sum_{I=1}^{n_{\chi}}   \bB^\chi_I \cdot  \bD^\chi_I
\end{equation}
with 
\begin{equation}
\bB^\chi_I = \left(\begin{matrix}
0 & N^{\chi}_{I,1} & 0  & -N^{\chi}_{I,1} \\
-N^{\chi}_{I,2} & 0  & N^{\chi}_{I,1} & 0 \\
 \end{matrix}\right)\,.  \quad \Curl \tilde{\Bchi} = \left(\begin{matrix}
\Curl \chi_{13} \\ 
\Curl \chi_{23} \\
 \end{matrix}\right)\,.
\end{equation}
Thus, we have 
\begin{equation}
\begin{aligned}
(\Delta \delta \Pi_u)_e = & \sum_I^{n_u}  \sum_J^{n_u}   (\delta \bd_I^u)^T  \underbrace{\int_{\B} (\bB_I^u)^T \cdot \tilde{\Ce} \cdot \bB_J^u  \; \textrm{d}V}_{\bK_{IJ}^{uu}} \Delta \bd_J^u\\
 & -  \sum_I^{n_u}  \sum_J^{n_\chi}  (\delta \bd_I^u)^T  \underbrace{ \int_{\B} (\bB_I^u)^T \cdot \tilde{\Ce} \cdot   \bN^\chi_J  \; \textrm{d}V}_{-\bK_{IJ}^{u\chi}} \Delta \bD^\chi_J \,, \\
 \end{aligned}
\end{equation}
and 
\begin{equation}
\begin{aligned}
(\Delta \delta \Pi_\chi)_e =& - \sum_I^{n_\chi}  \sum_J^{n_u}   (\delta \bD_I^\chi)^T  \underbrace{\int_{\B}  (\bN^\chi_I)^T  \cdot  \tilde{\Ce} \cdot \bB_J^u  \; \textrm{d}V}_{-\bK_{IJ}^{\chi u}}    \Delta \bd_J^u  \\
& + \sum_I^{n_\chi}  \sum_J^{n_\chi}   (\delta \bD_I^\chi)^T  \underbrace{\int_{\B}  (\bN^\chi_I)^T  \cdot (\tilde{\Ce} + \tilde{\mathbb{C}}_\textrm{micro}) \cdot  \bN_J^\chi   +  \mu \, l_c^2 (\bB_I^\chi)^T \cdot \bB_J^\chi  \;\; \textrm{d}V}_{\bK_{IJ}^{\chi\chi}} \Delta \bD_J^\chi =  0 \,,
 \end{aligned}
\end{equation}
and the element stiffness matrix reads 
\begin{equation}
\bK^e = \left(\begin{matrix}
\bK^{uu} &  \bK^{u\chi} \\ 
\bK^{\chi u} &  \bK^{\chi \chi} \\ 
\end{matrix}\right) =  
\left( \begin{array}{ccc|ccc}
\bK^{uu}_{11} & ... & \bK^{uu}_{1n_u} & \bK^{u \chi}_{11} & ... & \bK^{u \chi}_{1n_\chi}   \\ 
.... & .... & ... & .... & .... & ...   \\ 
\bK^{uu}_{n_u 1} & ... & \bK^{uu}_{n_u n_u} & \bK^{u \chi}_{n_u 1} & ... & \bK^{uu}_{n_u n_\chi}  \\ \hline
\bK^{\chi u}_{11} & ... & \bK^{\chi u}_{1 n_u} & \bK^{\chi \chi}_{1 1} & ... & \bK^{\chi \chi}_{1 n_\chi}  \\ 
.... & .... & ... & .... & .... & ...   \\ 
\bK^{\chi u}_{n_\chi 1} & ... & \bK^{\chi u}_{n_\chi n_u} & \bK^{\chi \chi}_{n_\chi 1} & ... & \bK^{\chi \chi}_{n_\chi  n_\chi}  \\ 
 \end{array} \right)\,.  
\end{equation}
For the tangential conforming finite elements, we have instead 
 \begin{equation}
\sym \tilde{\Bchi} =   \sum_{I=1}^{n_{\chi}}   \BPsi^\chi_I \cdot  \bd^\chi_I 
\end{equation}
with 
\begin{equation}
 \BPsi^\chi_I = \left( \begin{matrix}
 {\psi^\chi_{(1)}}_I  & 0 \\
0  &    {\psi^\chi_{(2)}}_I  \\
 {\psi^\chi_{(2)}}_I    &   {\psi^\chi_{(1)}}_I   \\
 \end{matrix} \right)\,, \quad \bd^\chi_I = \left( \begin{matrix} 
 d^\chi_{(1)I} \\
 d^\chi_{(2)I}
 \end{matrix} \right) 
\end{equation}
where $ {\psi^\chi_{(1)}}_I \textrm{ and }  {\psi^\chi_{(2)}}_I$ are the components of the vectorial shape function $\Bpsi_I$. 
The curl of the micro-distortion field is defined for the tangential conforming elements  for the 2-dimensional case as
\begin{equation}
\Curl \tilde{\Bchi} =  \sum_{I=1}^{n_{\chi}}   \bar{\bB}^\chi_I \cdot  \bd^\chi_I
\end{equation}
with 
\begin{equation}
  \bar{\bB}^\chi_I = \left(\begin{matrix} \Curl^{2D}_\bX {\Bpsi^\chi_I} & 0 \\ 
  0 & \Curl^{2D}_\bX {\Bpsi^\chi_I} 
  \end{matrix}
 \right). 
\end{equation}
and we have instead 
\begin{equation} 
\begin{aligned}
\bK_{IJ}^{u\chi} &= \int_{\B} (\bB_I^u)^T \cdot \tilde{\Ce} \cdot   \BPsi^\chi_I  \; \textrm{d}V\,, \\ 
\bK_{IJ}^{\chi u} &= \int_{\B} (\BPsi^\chi_I)^T \cdot \tilde{\Ce} \cdot   \bB_J^u \; \textrm{d}V\,, \\ 
\bK_{IJ}^{\chi \chi} &= \int_{\B}  (\BPsi^\chi_I)^T  \cdot (\tilde{\Ce} + \tilde{\mathbb{C}}_\textrm{micro}) \cdot  \BPsi_J^\chi   +  \mu \, l_c^2 (\bar{\bB}_I^\chi)^T \cdot \bar{\bB}_J^\chi  \;\; \textrm{d}V\,.\\ 
\end{aligned}
\end{equation}
%=========================================================================
\sect{\hspace{-5mm}. Examples}


\ssect{\hspace{-5mm}. Interface between two different materials} 
\label{bvp:2}
Two blocks of different materials are set with an vertical interface between, see Figure \ref{Figure:Geo2}. \\
\begin{figure}[ht]
\center
	\unitlength=1mm
	\begin{picture}(200,55)
	\put(35,0){\def\svgwidth{10cm}{\small\input{figures/example2_geo.eps_tex}}}
	\end{picture}
	\caption{Second example geometry. Inspection line can be seen in red color and the inspection line can be seen in red color. }
	\label{Figure:Geo2}
\end{figure} 

The bottom edge is fixed on both directions $u_x = u_y = 0$ and we apply a displacement to the upper edge as $u_x = u_y = 0.02$. For the distortion field, we apply for the both bottom and upper edges $\bd^\chi_x = \bd^\chi_y = 0$ for the elements with tangential conforming shape functions (T2NT1, Q2NQ1, T2NT2 and Q2NQ2) which is equivalent to enforce $\bD^\chi_{xx} = \bD^\chi_{yx} = 0$ for the element with Lagrange shape functions (T2T1).   \\

Micromorphic model parameters: \\
Characteristic length $l_c =1$, and  the rest of the material moduli are explained in A. 7 with $\alpha = 1$, $\phi =0.5$ and the following: \\
{\bf Domain 1}: \\
First Material: Young's modulus $E_1= 1000$ and  Poisson's ratio
$\nu_1 =  0.2$\,. \\
Second Material: Young's modulus $E_2= 3000$ and  Poisson's ratio $\nu_2 =  0.2$\,. \\
{\bf Domain 2}: \\
First Material: Young's modulus $E_1= 2000$ and  Poisson's ratio
$\nu_1 =  0.2$\,. \\
Second Material: Young's modulus $E_2= 6000$ and  Poisson's ratio $\nu_2 =  0.2$\,. \\

Results:
\FloatBarrier
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/2_Q2NQ1_u1.png}
			\caption{$u_x$}
     \end{subfigure}
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/2_Q2NQ1_u2.png}
			\caption{$u_y$}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/2_Q2NQ1_chi11.png}
			\caption{$\chi_{xx}$}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/2_Q2NQ1_chi22.png}
			\caption{$\chi_{yy}$}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/2_Q2NQ1_chi12.png}
			\caption{$\chi_{xy}$}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/2_Q2NQ1_chi21.png}
			\caption{$\chi_{yx}$}
     \end{subfigure}
        \caption{The Displacement  and $\Bchi$ components of the interface example using Q2NQ1}
\end{figure}


\begin{figure}[ht]
	\unitlength=1mm
	\center
	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/chiyx_convergence_T2T1.eps}
         \put(-35,-2){$x$}
	\caption{T2T1}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/chiyx_convergence_T2NT1.eps}
         \put(-35,-2){$x$}
	\caption{T2NT1}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/chiyx_convergence_Q2NQ1.eps}
         \put(-35,-2){$x$}
	\caption{Q2NQ1}
		  \end{subfigure}
		  	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/chiyx_convergence_T2NT2.eps}
         \put(-35,-2){$x$}
	\caption{T2NT2}
		  \end{subfigure}
		  	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/chiyx_convergence_Q2NQ2.eps}
         \put(-35,-2){$x$}
	\caption{Q2NQ2}
		  \end{subfigure}		  
		  	\caption{$\chi_{yx}$ along inspection line using different mesh densities}
\end{figure} 


\begin{figure}[ht]
	\unitlength=1mm
	\center
	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/2_inspectionline_T2T1.eps}
         \put(-35,-2){$x$}
	\caption{T2T1 with 103684 elements}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/2_inspectionline_T2NT1.eps}
         \put(-35,-2){$x$}
	\caption{T2NT1 with 12996 elements}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/2_inspectionline_Q2NQ1.eps}
         \put(-35,-2){$x$}
	\caption{Q2NQ1 with 13122 elements}
		  \end{subfigure}
		  	  	  \begin{subfigure}[b]{0.49\textwidth}
       \includegraphics[width=\textwidth]{figures/2_inspectionline_T2NT2.eps}
         \put(-35,-2){$x$}
	\caption{T2NT2 with 484 elements}
		  \end{subfigure}
		  	  	  \begin{subfigure}[b]{0.49\textwidth}
       \includegraphics[width=\textwidth]{figures/2_inspectionline_Q2NQ2.eps}
         \put(-35,-2){$x$}
	\caption{Q2NQ2 with 450 elements}
		  \end{subfigure}		  
		  	\caption{$\Bchi$ components along inspection line for the converged results}
\end{figure} 
\FloatBarrier

\FloatBarrier

\newpage
\ssect{\hspace{-5mm}.Circle with a hole} 
We set a circle with a circular hole inside, see Figure \ref{Figure:Geo4}. The hole is located at the center with a radius $r_0 =2$ and the outer radius of $r_1=25$.
\begin{figure}[ht]
\center
	\unitlength=1mm
	\begin{picture}(150,100)
	\put(35,0){\def\svgwidth{8cm}{\small\input{figures/example4_geo.eps_tex}}}
	\end{picture}
	\caption{Circle with a circular hole boundary value problem }
	\label{Figure:Geo4}
\end{figure} \\
The r.m.m material moduli are obtained as in A. 7. We use  $\Lc = 5$, $ \alpha = 0$ and  $\phi =0.5$ if nothing else is mentioned. The resting parameters read: \\
First Material: Young's modulus $E_1= 1000$ and  Poisson's ratio and  $\nu_1 =  0.2$ \\
Second Material: Young's modulus $E_2= 3000$ and  Poisson's ratio $\nu_2 =  0.2$


\begin{center}
\begin{table}[ht]
\begin{tabular}{|c|c|}
\cline{1-2}
Boundary condition &  position    \\  \cline{1-2}
$ \bd^u=\bzero$ &  $x^2 + y^2 = r_0^2 = 4$   \\ \cline{1-2}
$ d^u_x= - \frac{\Delta}{r_2} y,  d^u_y=\frac{\Delta}{r_2} x$ &  $x^2 + y^2 =r_2^2 = 25$   \\ \cline{1-2}
 $\Bchi \cdot \bt = \Grad \bu \cdot \bt$ & $\partial \B$ \\ \cline{1-2}
\end{tabular}
\end{table}
\end{center}
 with $ \Delta = 0.01$.  \\
 
 \textbf{Convergence:} \\


\begin{figure}[ht]
	\unitlength=1mm
	\center
	  \begin{subfigure}[b]{0.95\textwidth}
         \includegraphics[width=\textwidth]{figures/convergence_T2T1.eps}
	\caption{T2T1}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.95\textwidth}
         \includegraphics[width=\textwidth]{figures/convergence_T2NT1.eps}
	\caption{T2TN1}
		  \end{subfigure}
		  	  	  \begin{subfigure}[b]{0.95\textwidth}
         \includegraphics[width=\textwidth]{figures/convergence_T2NT2.eps}
	\caption{T2TN2 }
		  \end{subfigure}
		  	\caption{Convergence study: the non-vanishing components of $\Bchi$ along the radius using different mesh densities. }
\end{figure}  
 \FloatBarrier

  \textbf{$\Lc$ study} \\

for $\Lc \rightarrow \infty$, we obtain $\Grad \bu \cdot \bt = \Bchi \cdot \bt$. However, Lagrange element results are inconsistent  for $\Lc \rightarrow \infty$. 

\begin{figure}[ht]
	\unitlength=1mm
	\center
	  \begin{subfigure}[b]{0.75\textwidth}
         \includegraphics[width=\textwidth]{figures/lc_study_T2T1.eps}
	\caption{T2T1}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.75\textwidth}
         \includegraphics[width=\textwidth]{figures/lc_study_T2NT1.eps}
	\caption{T2TN1}
		  \end{subfigure}
		  	  	  \begin{subfigure}[b]{0.75\textwidth}
         \includegraphics[width=\textwidth]{figures/lc_study_T2NT2.eps}
	\caption{T2TN2 }
		  \end{subfigure}
		  	\caption{The non-vanishing components of $\Bchi$ and $\bH= \Grad \bu $ using 30786 elements with different values for $\Lc$.} 
\end{figure}  

\FloatBarrier

  \textbf{Force and moment stresses:} \\
$\Bsigma = \Ce : \symb{ \Grad\bu - \Bchi} + \Cc  : \skewb{ \Grad\bu - \Bchi}\,, \quad \bM =  \mu \, \Lc^2 \,  \textrm{Curl} \Bchi\,.$ \\ 
For $\Lc \rightarrow 0$, we get $\Bsigma = \Bsigma^\textrm{macro}$ and $\bM \rightarrow \bzero$. 
For $\Lc \rightarrow \infty$, we get $\Bsigma \rightarrow \bzero$ and moment stress is $\bM$ is at its highest level. 

\begin{figure}[ht]
\center
	\unitlength=1mm
	\begin{picture}(200,80)
	         \includegraphics[width=\textwidth]{figures/force_stress.eps}
	\end{picture}
	\caption{The non-vanishing components of the symmetric force stress $\Bsigma$ using 30786 T2NT1 elements with different values of $\L_{c}$ compared to linear elasticity with elasticity tensors $\Cmicro$ and $\Cmacro$. }
\end{figure} 

\begin{figure}[ht]
\center
	\unitlength=1mm
	\begin{picture}(200,80)
	         \includegraphics[width=\textwidth]{figures/moment_stress.eps}
	\end{picture}
	\caption{The only non-vanishing component of the moment stress $M_{r z}$  using 30786 T2NT1 elements with different values of $\L_{c}$. }
\end{figure} 

\begin{figure}[ht]
\center
	\unitlength=1mm
	\begin{picture}(200,120)
	         \includegraphics[width=\textwidth]{figures/Potential_study.eps}
	\end{picture}
	\caption{The potential of the relaxed micromorphic model along the radius compared to linear elasticity with elasticity tensors $\Cmicro$ and $\Cmacro$. }
\end{figure} 

\FloatBarrier

\begin{figure}[ht]
	\unitlength=1mm
	\center
	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/elastic_energy_study.eps}
	\caption{$ \psi_\textrm{e} = \frac{1}{2} \symb{ \nabla \bu - \Bchi} : \Ce : \symb{ \nabla \bu - \Bchi}$  }
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/micro_energy_study.eps}
	\caption{$ \psi_\textrm{micro} = \frac{1}{2} \sym \Bchi : \Cmicro: \sym \Bchi $  }
		  \end{subfigure}
		  	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/curvature_energy_study.eps}
	\caption{$\psi_\textrm{curvature} = \frac{1}{2} \mu \, \Lc^2 \, \textrm{Curl} \Bchi : \IL :\textrm{Curl} \Bchi$ }
		  \end{subfigure}
		  	\caption{The different parts of the potential of the relaxed micromorphic model along the radius using different values of the characteristic  length. Black arrows indicates the effects of increasing the  characteristic  length $L_c$.}
\end{figure}  
 \FloatBarrier
 
\newpage
\ssect{\hspace{-5mm}.Two rings} 
We set two rings consisting of two different combinations of materials (domains), see Figure \ref{Figure:Geo3}. A circular hole at the center has a radius of $r_0 =2$, the inner ring has an inner radius of $r_0 =2$ and outer radius of $r1=10$, and the outer radius has an inner radius of $r_1=10$ and outer radius of $r_2=25$.
\begin{figure}[ht]
\center
	\unitlength=1mm
	\begin{picture}(150,75)
	\put(35,0){\def\svgwidth{8cm}{\small\input{figures/example3_geo.eps_tex}}}
	\end{picture}
	\caption{Third example geometry. Three inspection lines can be seen in red color. }
	\label{Figure:Geo3}
\end{figure} \\
The r.m.m material moduli are obtained as in A. 7. We use $l_c = 1$, $ \alpha = 0$ and  $\phi =0.5$ if nothing else is mentioned. The resting parameters read:\\
{\bf Domain 1} \\
First Material: Young's modulus $E_1= 1000$ and  Poisson's ratio
$\nu_1 =  0.2$\,. shear modulus $G_1 = 416.67$ \\
Second Material: Young's modulus $E_2= 3000$ and  Poisson's ratio $\nu_2 =  0.2$\,.  shear modulus $G_2 = 1250$  \\
{\bf Domain 2} \\
First Material: Young's modulus $E_1= f*1000$ and  Poisson's ratio
$\nu_1 =  0.2$\,. shear modulus $G_1 = f*416.67$ \\
Second Material: Young's modulus $E_2= f*3000$ and  Poisson's ratio $\nu_2 =  0.2$\,. shear modulus $G_1 = f*1250$ \\ 
$f=2$ if nothing else is mentioned. 



\newpage
\sssect{Case 1: shear Loading\\} 

Boundary conditions:
\begin{center}
\begin{table}[ht]
\begin{tabular}{|c|c|}
\cline{1-2}
Boundary condition &  position    \\  \cline{1-2}
$ \bd^u=\bzero$ &  $x^2 + y^2 = r_0^2 = 4$   \\ \cline{1-2}
$ d^u_x= - \frac{\Delta}{r_2} y,  d^u_y=\frac{\Delta}{r_2} x$ &  $x^2 + y^2 =r_2^2 = 25$   \\ \cline{1-2}
$\Bchi \cdot \bt=0$ &  $x^2 + y^2 = r_0^2 = 2$ and   $x^2 + y^2 = r_2^2 =25$ \\ \cline{1-2}
\end{tabular}
\end{table}
\end{center}
where $ \Delta = 0.01$.  \\

Results: \\
\FloatBarrier

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/3_Q2NQ1_u1.png}
			\caption{$u_x$ using Q2NQ1}
     \end{subfigure}
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/3_Q2NQ1_u2.png}
			\caption{$u_y$ using Q2NQ1}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/3_Q2NQ1_chi11.png}
			\caption{$\chi_{xx}$ using Q2NQ1}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/3_Q2NQ1_chi22.png}
			\caption{$\chi_{yy}$ using Q2NQ1}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/3_Q2NQ1_chi12.png}
			\caption{$\chi_{xy}$ using Q2NQ1}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/3_Q2NQ1_chi21.png}
			\caption{$\chi_{yx}$ using Q2NQ1}
     \end{subfigure}
        \caption{The Displacement  and $\Bchi$ components of the rings example }
\end{figure}
\FloatBarrier

{\bf $\Bchi$ in polar coordinates:} 
We could obtain the polar components of $\Bchi$ in the two dimensional case simply as 
\begin{equation}
\Bchi^\textrm{P} =  
 \left[ \begin{array}{ccc}
\Bchi_{rr} & \Bchi_{r \theta} \\
 \Bchi_{\theta r} & \Bchi_{\theta \theta}\\
\end{array}\right]  = \bR^T \cdot \Bchi \cdot \bR\,,
\end{equation}
where $\bR$ is the rotation matrix which reads for the two-dimensional case
\begin{equation}
\bR =
 \left[ \begin{array}{ccc}
 \cos(\theta) & -\sin(\theta)\\
\sin(\theta) & \cos(\theta)\\
\end{array}\right] 
\end{equation}
where $\cos(\theta) = x/\sqrt(x^2+y^2)$ and $\sin(\theta) = y/\sqrt(x^2+y^2)$ 


\begin{figure}[ht]
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/3_Q2NQ1_chi_r_theta_cc=0.png}
        \caption{$\chi_{r \theta}$ using Q2NQ1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/3_Q2NQ1_chi_theta_r_cc=0.png}
			\caption{$\chi_{\theta r}$ using Q2NQ1}
     \end{subfigure}
        \caption{The non-vanishing polar components of $\Bchi$ for the rings example using Q2NQ1 with $\alpha=0$. }
\end{figure}

\begin{figure}[ht]
	\unitlength=1mm
	\center
	  \begin{subfigure}[b]{0.75\textwidth}
         \includegraphics[width=\textwidth]{figures/3_T2NT1_T2NT2.eps}
         \put(-35,-2){$x$}
	\caption{T2NT1 and T2NT2 using  1666 elements  }
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.75\textwidth}
         \includegraphics[width=\textwidth]{figures/3_Q2NQ1_Q2NQ2.eps}
         \put(-35,-2){$x$}
	\caption{Q2NQ1 and Q2NQ2 using  1652 elements }
		  \end{subfigure}
		  	  	  \begin{subfigure}[b]{0.75\textwidth}
         \includegraphics[width=\textwidth]{figures/3_T2T1.eps}
         \put(-35,-2){$x$}
	\caption{T2T1 using 31412 elements }
		  \end{subfigure}
		  	\caption{The non-vanishing polar components of $\Bchi$ along the radius.}
\end{figure} 



\begin{figure}[ht]
\center
	\unitlength=1mm
	\begin{picture}(200,90)
	\put(0,0){\def\svgwidth{16cm}{\small\input{figures/3_Q2NQ1_line_f_study.eps_tex}}}
	\end{picture}
	\caption{The polar components of $\Bchi$ along the diameter using Q2NQ1 and different value for $f$. $\chi_{r \theta}$ is in red and $\chi_{ \theta r}$ in blue.  }
\end{figure} 


\FloatBarrier
We set $lc \rightarrow 0$ (very large sample), the relaxed micromorphic model strong forms turn to 
\eb
\Divb{\IC_{e} : \symb{ \Grad \bu - \Bchi} + \IC_{c} : \skewb{ \Grad \bu - \Bchi}} = \bbf 
\label{eq:stress1}
\ee
and 
\eb
\IC_{e} : \symb{ \Grad \bu - \Bchi} + \IC_{c} : \skewb{ \Grad \bu - \Bchi} 
- \IC_\textrm{micro} : \sym \Bchi = \bzero  
\ee
which result into the macroscopic linear elastic response with the effective macroscopic elasticity tensor $\IC_\textrm{macro}
$
\eb
\Divb{\IC_\textrm{macro} : \symb{ \Grad \bu}} = \bbf 
\label{eq:stress2}
\ee
where $\IC_\textrm{macro}$ is given as 
\eb
\IC_\textrm{macro} = \left( \IC_\textrm{macro}^{-1} + \IC_\textrm{e}^{-1} \right)^{-1} 
\ee

\begin{figure}[ht]
\center
         \includegraphics[width=0.75\textwidth]{figures/test_lc_0.eps}
	\caption{The non-vanishing components of $\Bsigma$ along the radius using 30640 elements of T2NT2 with the stress measurement in Eq. \ref{eq:stress1} or using 30640 linear elastic elements (T2) with the stress measurement in Eq. \ref{eq:stress2}.}
\end{figure} 


\FloatBarrier
\newpage
\sssect{\hspace{-5mm} Case 2: normal loading\\} 
\vspace{1 cm}
Boundary conditions:\\ 
\begin{center}
\begin{table}[ht]
\begin{tabular}{|c|c|}
\cline{1-2}
Boundary condition &  position    \\  \cline{1-2}
$ \bd^u=\bzero$ &  $x^2 + y^2 = r_0^2 = 4$   \\ \cline{1-2}
$ d^u_x=  \frac{\Delta}{r_2} x,  d^u_y=\frac{\Delta}{r_2} y$ &  $x^2 + y^2 =r_2^2 = 25$   \\ \cline{1-2}
$ \Bchi \cdot \bt = \bzero$ &  $x^2 + y^2 = r_0^2 = 2$ and   $x^2 + y^2 = r_2^2 =25$ \\ \cline{1-2}
\end{tabular}
\end{table}
\end{center}
where $ \Delta = 0.01$.  \\


Results: \\

$\alpha$ has no effects in this example since  $\skewb{ \Grad \bu - \Bchi}$  vanishes (only normal components are active) .

\begin{figure}[ht]
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/3_Q2NQ1_chi_r_r_cc=0.png}
        \caption{$\chi_{r r}$ using Q2NQ1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/3_Q2NQ1_chi_theta_theta_cc=0.png}
			\caption{$\chi_{\theta \theta}$ using Q2NQ1}
     \end{subfigure}
        \caption{The non-vanishing polar components of $\Bchi$ for the rings example using Q2NQ1.  }
\end{figure}


\begin{figure}[ht]
	\unitlength=1mm
	\center
	  \begin{subfigure}[b]{0.75\textwidth}
         \includegraphics[width=\textwidth]{figures/3_T2NT1_T2NT2_normal.eps}
         \put(-35,-2){$x$}
	\caption{T2NT1 and T2NT2 using  1666 elements  }
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.75\textwidth}
         \includegraphics[width=\textwidth]{figures/3_Q2NQ1_Q2NQ2_normal.eps}
         \put(-35,-2){$x$}
	\caption{Q2NQ1 and Q2NQ2 using  1652 elements }
		  \end{subfigure}
		  		  	  	  \begin{subfigure}[b]{0.75\textwidth}
         \includegraphics[width=\textwidth]{figures/3_T2T1_normal.eps}
         \put(-35,-2){$x$}
	\caption{T2T1 using 31412 elements }
		  \end{subfigure}
		  	\caption{The non-vanishing polar components of $\Bchi$ along the radius.}
\end{figure} 

\begin{figure}[ht]
\center
	\unitlength=1mm
	\begin{picture}(200,90)
	\put(0,0){\def\svgwidth{16cm}{\small\input{figures/3_Q2NQ1_line_f_study_normal.eps_tex}}}
	\end{picture}
	\caption{The polar components of $\Bchi$ along the diameter using Q2NQ1 with different values for $f$. }
\end{figure} 

\FloatBarrier

\sssect{Case 3: shear Loading with $\Bchi \cdot \bt = \Grad \bu \cdot \bt$ on the boundary \\} 

\begin{center}
\begin{table}[ht]
\begin{tabular}{|c|c|}
\cline{1-2}
Boundary condition &  position    \\  \cline{1-2}
$ \bd^u=\bzero$ &  $x^2 + y^2 = r_0^2 = 4$   \\ \cline{1-2}
$ d^u_x= - \frac{\Delta}{r_2} y,  d^u_y=\frac{\Delta}{r_2} x$ &  $x^2 + y^2 =r_2^2 = 25$   \\ \cline{1-2}
 $\Bchi \cdot \bt = \Grad \bu \cdot \bt$ & $\partial \B$ \\ \cline{1-2}
\end{tabular}
\end{table}
\end{center}
 with $ \Delta = 0.01$.  \\

\begin{figure}[ht]
\center
         \includegraphics[width=0.75\textwidth]{figures/Image_Lc_study.eps}
	\caption{$\chi_{r \theta}$ and $u_{r,\theta}$  along the radius using different values of the characteristic length $L_c$.    }
\end{figure} 
\FloatBarrier
\sssect{Case 4: $\Bchi \cdot \bt =  \Grad \bu \cdot \bt$ on a part of the outer boundary with $L_c = 100000$ \\} 

We set on the inner boundary $\Bchi \cdot \bt =  \Grad \bu \cdot \bt$ but on the inner boundary, we set $\Bchi \cdot \bt =  \Grad \bu \cdot \bt$ on part of it. 

\begin{figure}[ht]
\center
	\unitlength=1mm
	\begin{picture}(150,100)
	\put(10,0){\def\svgwidth{12cm}{\small\input{figures/example3_geo_part_boundary.eps_tex}}}
	\end{picture}
	\caption{$\Bchi \cdot \bt =  \Grad \bu \cdot \bt$ is enforced on the full outer boundary for case 1, one half of the boundary in case 2, one quarter of the boundary for case  3 and one eighth of the boundary for case 4. Inspection line can be seen in red color.  }
\end{figure} 

\begin{figure}[ht]
\center
         \includegraphics[width=0.75\textwidth]{figures/Image_boundary_study.eps}
	\caption{Non-vanishing $\Bchi$ and $\Grad \bu$ components  along the line $y=0$ with $\Bchi \cdot \bt =  \Grad \bu \cdot \bt$ enforced on the full or parts of the outer boundary. }
\end{figure} 

\FloatBarrier
\newpage
\sssect{Case 5: additional penalty term in the energy $W_p = \frac{w}{2} \skew \Bchi :  \skew \Bchi$ \\} 

\begin{center}
\begin{table}[ht]
\begin{tabular}{|c|c|}
\cline{1-2}
Boundary condition &  position    \\  \cline{1-2}
$ \bd^u=\bzero$ &  $x^2 + y^2 = r_0^2 = 4$   \\ \cline{1-2}
$ d^u_x= - \frac{\Delta}{r_2} y,  d^u_y=\frac{\Delta}{r_2} x$ &  $x^2 + y^2 =r_2^2 = 25$   \\ \cline{1-2}
\end{tabular}
\end{table}
\end{center}

 with $ \Delta = 0.01$.  \\
Results: Q2NQ2 element 

\begin{center}
\begin{table}[ht]
\begin{tabular}{|c|c|c|}
\cline{1-3}
w &  number of zero eigenvalues  & $\frac{1}{V} \int_{\B}  |\chi_{xy} - \chi_{yx} | \; \textrm{d}V $\\  \cline{1-3}
0 & 4 & $6,7 \cdot 10^{-4}$  \\ \cline{1-3}
1 & 3  & $6,2 \cdot 10^{-4}$  \\ \cline{1-3}
10 & 3 & $4,2 \cdot 10^{-4}$   \\ \cline{1-3}
10 & 3 & $1,6 \cdot 10^{-4}$  \\ \cline{1-3}
$10^2$ &  3 & $5,1 \cdot 10^{-5}$  \\ \cline{1-3}
$10^3$ & 3  & $1,3 \cdot 10^{-5}$ \\ \cline{1-3}
$10^4$ & 3  & $2,45 \cdot 10^{-6}$  \\ \cline{1-3}
$10^5$ & 3  & $6,7 \cdot 10^{-7}$  \\ \cline{1-3}
$10^6$ & 3 & $3,3 \cdot 10^{-7}$  \\ \cline{1-3}
$10^7$ & 3  & $1,14 \cdot 10^{-7}$ \\ \cline{1-3}
$10^8$ & 3  & $2,61 \cdot 10^{-8}$ \\ \cline{1-3}
$10^9$ & 3 & $4,39 \cdot 10^{-9}$ \\ \cline{1-3}
\end{tabular}
\end{table}
\end{center}


If we set $\Cc \neq \bzero$ ($\alpha \neq 0$), then we get 3 zero eigenvalues with or without the penalty term!   \\
All eigenvalues are positive or zeros till $w \approx 10^{15}$. 

\begin{figure}[ht]
\center
         \includegraphics[width=0.95\textwidth]{figures/Image_Lc_study_alpha=0.eps}
	\caption{Non vanishing components of $\Bchi$ and $ \Grad \bu$ along the radius using different values of the characteristic length $L_c$ with $\Cc =  \bzero$ and $\Bchi \cdot \bt = \Grad \bu \cdot \bt$ and without penalty.  }
\end{figure} 

\begin{figure}[ht]
\center
         \includegraphics[width=0.95\textwidth]{figures/Image_Lc_study_alpha=0_w=1000}
	\caption{Non vanishing components of $\Bchi$ and $ \Grad \bu$ along the radius using different values of the characteristic length $L_c$, $\Cc =  \bzero$ and $w=1000$. No boundary conditions are enforced for $\Bchi$. }
\end{figure} 

\begin{figure}[ht]
\center
         \includegraphics[width=0.95\textwidth]{figures/Image_Lc_study_alpha=1_w=1000}
	\caption{Non vanishing components of $\Bchi$ and $ \Grad \bu$ along the radius using different values of the characteristic length $L_c$, $\Cc =  2 \mu_\textrm{Reuss} \tilde{\II} $ and $w=1000$. No boundary conditions are enforced for $\Bchi$. }
\end{figure} 

\begin{figure}[ht]
\center
         \includegraphics[width=0.95\textwidth]{figures/Image_Lc_study_alpha=1.eps}
	\caption{Non vanishing components of $\Bchi$ and $ \Grad \bu$ along the radius using different values of the characteristic length $L_c$ with $\Cc =  2 \mu_\textrm{Reuss} \tilde{\II} $. No boundary conditions for $\Bchi$ are enforced. }
\end{figure} 

\newpage
\FloatBarrier
\ssect{\hspace{-5mm} Shear boundary value problem}
The material moduli are obtained as in A. 7. We use $\phi =0.5$ if nothing else is mentioned. The resting parameters read:\\
First Material: Young's modulus $E_1= 1000$ and  Poisson's ratio
$\nu_1 =  0.2$\,. Shear modulus reads $G_1 = 416.67$ \\
Second Material: Young's modulus $E_2= 3000$ and  Poisson's ratio $\nu_2 =  0.2$\,.  Shear modulus reads $G_2 = 1250$  \\
We use $l=2, h=1$ and $\Delta = 0.02$. We discretize the problem using 20 x 10 elements.
\begin{figure}[ht]
\center
	\unitlength=1mm
	\begin{picture}(150,75)
	\put(10,0){\def\svgwidth{15cm}{\small\input{figures/shear_BVP.eps_tex}}}
	\end{picture}
	\caption{Shear boundary value problem. }
	\label{Figure:Geo3}
\end{figure} 
\newpage
\FloatBarrier
\sssect{\hspace{-5mm} $\Cc =  2 \mu_\textrm{Reuss} \tilde{\II} $}

\begin{figure}[ht]
	\unitlength=1mm
	\center
	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=0,001,all_boundaries_chit=Gradut,y=0,5.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=0.001$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=0,001,all_boundaries_without_the_upper_boundary_chit=Gradut,y=0,5.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=0.001$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B \backslash y=h$}
		  \end{subfigure}
	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1,all_boundaries_chit=Gradut,y=0,5.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1,all_boundaries_without_the_upper_boundary_chit=Gradut,y=0,5.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B \backslash y=h$}
		  \end{subfigure}
		  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1000,all_boundaries_chit=Gradut,y=0,5.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1000$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1000,all_boundaries_without_the_upper_boundary_chit=Gradut,y=0,5.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1000$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B \backslash y=h$}
		  \end{subfigure}
		  	\caption{$\Bchi$  and $\Grad \bu$ component along the line $y=h/2$.}
\end{figure} 


\begin{figure}[ht]
	\unitlength=1mm
	\center
		  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=0,001,all_boundaries_chit=Gradut,x=1.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=0.001$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=0,001,all_boundaries_without_the_upper_boundary_chit=Gradut,x=1.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=0,001$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B \backslash y=h$}
		  \end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
		  \includegraphics[width=\textwidth]{figures/Lc=1,all_boundaries_chit=Gradut,x=1.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1,all_boundaries_without_the_upper_boundary_chit=Gradut,x=1.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B \backslash y=h$}
		  \end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
		  \includegraphics[width=\textwidth]{figures/Lc=1000,all_boundaries_chit=Gradut,x=1.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1000$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1000,all_boundaries_without_the_upper_boundary_chit=Gradut,x=1.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1000$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B \backslash y=h$}
		  \end{subfigure}
		  	\caption{$\Bchi$  and $\Grad \bu$ component along the line $x=l/2$.}
\end{figure} 
\begin{figure}[ht]
	\unitlength=1mm
	\center
		  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=0,001,penalty=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=0.001$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1,penalty=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1$}
		  \end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
		  \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1000$}
		  \end{subfigure}
		  	\caption{$\Bchi$  and $\Grad \bu$ components along the line $y=h/2$ with $w=0$, no boundary conditions were enforced for $\Bchi$.}
\end{figure} 
\begin{figure}[ht]
	\unitlength=1mm
	\center
		  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=0,001,penalty=1.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=0.001$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1,penalty=1.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1$}
		  \end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
		  \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=1.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1000$}
		  \end{subfigure}
		  	\caption{$\Bchi$  and $\Grad \bu$ components along the line $y=h/2$ with $w=1$, no boundary conditions were enforced for $\Bchi$.}
\end{figure} 
\begin{figure}[ht]
	\unitlength=1mm
	\center
		  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=0,001,penalty=10.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=0.001$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1,penalty=10.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1$}
		  \end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
		  \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=10.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1000$}
		  \end{subfigure}
		  	\caption{$\Bchi$  and $\Grad \bu$ components along the line $y=h/2$ with $w=10$, no boundary conditions were enforced for $\Bchi$.}
\end{figure} 
\begin{figure}[ht]
	\unitlength=1mm
	\center
		  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=0,001,penalty=100.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=0.001$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1,penalty=100.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1$}
		  \end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
		  \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=100.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1000$}
		  \end{subfigure}
		  	\caption{$\Bchi$  and $\Grad \bu$ components along the line $y=h/2$ with $w=100$, no boundary conditions were enforced for $\Bchi$.}
\end{figure} 
\begin{figure}[ht]
	\unitlength=1mm
	\center
		  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=0,001,penalty=1000.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=0.001$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1,penalty=1000.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1$}
		  \end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
		  \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=1000.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1000$}
		  \end{subfigure}
		  	\caption{$\Bchi$  and $\Grad \bu$ components along the line $y=h/2$ with $w=1000$, no boundary conditions were enforced for $\Bchi$.}
\end{figure} 

\begin{figure}[ht]
	\unitlength=1mm
	\center
		  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=0,001,penalty=10000.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=0.001$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1,penalty=10000.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1$}
		  \end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
		  \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=10000.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1000$}
		  \end{subfigure}
		  	\caption{$\Bchi$  and $\Grad \bu$ components along the line $y=h/2$ with $w=10000$, no boundary conditions were enforced for $\Bchi$.}
\end{figure} 

\begin{figure}[ht]
	\unitlength=1mm
	\center
		  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=0,001,penalty=100000.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=0.001$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1,penalty=100000.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1$}
		  \end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
		  \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=100000.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1000$}
		  \end{subfigure}
		  	\caption{$\Bchi$  and $\Grad \bu$ components along the line $y=h/2$ with $w=100000$, no boundary conditions were enforced for $\Bchi$.}
\end{figure} 

\begin{figure}[ht]
	\unitlength=1mm
	\center
		  	  \begin{subfigure}[b]{0.33\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=0.eps}
         \put(-35,-2){$x$}
	\caption{$w=0$}
		  \end{subfigure}
\begin{subfigure}[b]{0.33\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1,penalty=1.eps}
         \put(-35,-2){$x$}
	\caption{$w=1$}
		  \end{subfigure}
		  	  \begin{subfigure}[b]{0.33\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=10.eps}
         \put(-35,-2){$x$}
	\caption{$w=10$}
		  \end{subfigure}
		  	  \begin{subfigure}[b]{0.33\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=100.eps}
         \put(-35,-2){$x$}
	\caption{$w=100$}
		  \end{subfigure}
			  	  \begin{subfigure}[b]{0.33\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=1000.eps}
         \put(-35,-2){$x$}
	\caption{$w=1000$}
		  \end{subfigure}
		  	  \begin{subfigure}[b]{0.33\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=10000.eps}
         \put(-35,-2){$x$}
	\caption{$w=10000$}
		  \end{subfigure}
\begin{subfigure}[b]{0.33\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=100000.eps}
         \put(-35,-2){$x$}
	\caption{$w=100000$}
		  \end{subfigure}
		  	\caption{$\Bchi$  and $\Grad \bu$ components along the line $y=h/2$ with different values for $w$ and $L_c=1000$, no boundary conditions were enforced for $\Bchi$.}
\end{figure} 

\newpage
\FloatBarrier
\sssect{\hspace{-5mm} $\Cc =  \bzero $}
\begin{figure}[ht]
	\unitlength=1mm
	\center
	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=0,001,all_boundaries_chit=Gradut,y=0,5_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=0.001$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=0,001,all_boundaries_without_the_upper_boundary_chit=Gradut,y=0,5_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=0.001$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B \backslash y=h$}
		  \end{subfigure}
	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1,all_boundaries_chit=Gradut,y=0,5_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1,all_boundaries_without_the_upper_boundary_chit=Gradut,y=0,5_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B \backslash y=h$}
		  \end{subfigure}
		  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1000,all_boundaries_chit=Gradut,y=0,5_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1000$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1000,all_boundaries_without_the_upper_boundary_chit=Gradut,y=0,5_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1000$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B \backslash y=h$}
		  \end{subfigure}
		  	\caption{$\Bchi$  and $\Grad \bu$ component along the line $y=h/2$.}
\end{figure} 


\begin{figure}[ht]
	\unitlength=1mm
	\center
		  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=0,001,all_boundaries_chit=Gradut,x=1_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=0.001$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=0,001,all_boundaries_without_the_upper_boundary_chit=Gradut,x=1_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=0,001$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B \backslash y=h$}
		  \end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
		  \includegraphics[width=\textwidth]{figures/Lc=1,all_boundaries_chit=Gradut,x=1_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1,all_boundaries_without_the_upper_boundary_chit=Gradut,x=1_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B \backslash y=h$}
		  \end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
		  \includegraphics[width=\textwidth]{figures/Lc=1000,all_boundaries_chit=Gradut,x=1_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1000$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1000,all_boundaries_without_the_upper_boundary_chit=Gradut,x=1_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1000$, $\Grad \bu \cdot \bt = \Bchi \cdot \bt$ on $\partial \B \backslash y=h$}
		  \end{subfigure}
		  	\caption{$\Bchi$  and $\Grad \bu$ component along the line $x=l/2$.}
\end{figure} 

\begin{figure}[ht]
	\unitlength=1mm
	\center
		  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=0,001,penalty=0_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=0.001$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1,penalty=0_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1$}
		  \end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
		  \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=0_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1000$}
		  \end{subfigure}
		  	\caption{$\Bchi$  and $\Grad \bu$ components along the line $y=h/2$ with $w=0$, no boundary conditions were enforced for $\Bchi$.}
\end{figure} 

\begin{figure}[ht]
	\unitlength=1mm
	\center
		  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=0,001,penalty=1_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=0.001$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1,penalty=1_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1$}
		  \end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
		  \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=1_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1000$}
		  \end{subfigure}
		  	\caption{$\Bchi$  and $\Grad \bu$ components along the line $y=h/2$ with $w=1$, no boundary conditions were enforced for $\Bchi$.}
\end{figure} 


\begin{figure}[ht]
	\unitlength=1mm
	\center
		  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=0,001,penalty=10_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=0.001$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1,penalty=10_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1$}
		  \end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
		  \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=10_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1000$}
		  \end{subfigure}
		  	\caption{$\Bchi$  and $\Grad \bu$ components along the line $y=h/2$ with $w=10$, no boundary conditions were enforced for $\Bchi$.}
\end{figure} 


\begin{figure}[ht]
	\unitlength=1mm
	\center
		  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=0,001,penalty=100_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=0.001$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1,penalty=100_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1$}
		  \end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
		  \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=100_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1000$}
		  \end{subfigure}
		  	\caption{$\Bchi$  and $\Grad \bu$ components along the line $y=h/2$ with $w=100$, no boundary conditions were enforced for $\Bchi$.}
\end{figure} 

\begin{figure}[ht]
	\unitlength=1mm
	\center
		  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=0,001,penalty=1000_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=0.001$}
		  \end{subfigure}
	  	  \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1,penalty=1000_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1$}
		  \end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
		  \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=1000_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1000$}
		  \end{subfigure}
		  	\caption{$\Bchi$  and $\Grad \bu$ components along the line $y=h/2$ with $w=1000$, no boundary conditions were enforced for $\Bchi$.}
\end{figure} 


\begin{figure}[ht]
	\unitlength=1mm
	\center
		  	  \begin{subfigure}[b]{0.33\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=0_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$w=0$}
		  \end{subfigure}
\begin{subfigure}[b]{0.33\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1,penalty=1_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$w=1$}
		  \end{subfigure}
		  	  \begin{subfigure}[b]{0.33\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=10_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$w=10$}
		  \end{subfigure}
		  	  \begin{subfigure}[b]{0.33\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=100_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$w=100$}
		  \end{subfigure}
			  	  \begin{subfigure}[b]{0.33\textwidth}
         \includegraphics[width=\textwidth]{figures/Lc=1000,penalty=1000_alpha=0.eps}
         \put(-35,-2){$x$}
	\caption{$w=1000$}
		  \end{subfigure}
		  	\caption{$\Bchi$  and $\Grad \bu$ components along the line $y=h/2$ with different values for $w$ and $L_c=1000$, no boundary conditions were enforced for $\Bchi$.}
\end{figure} 

\FloatBarrier
\ssect{\hspace{-5mm} Bending boundary value problem}
The material moduli are obtained as in A. 7. We use $\phi =0.5$ if nothing else is mentioned. The resting parameters read:\\
First Material: Young's modulus $E_1= 1000$ and  Poisson's ratio
$\nu_1 =  0.2$\,. Shear modulus reads $G_1 = 416.67$ \\
Second Material: Young's modulus $E_2= 3000$ and  Poisson's ratio $\nu_2 =  0.2$\,.  Shear modulus reads $G_2 = 1250$  \\
We use $l=2, h=1$ and $q = 1$. We discretize the problem using 40 x 20 elements.

\begin{figure}[ht]
\center
	\unitlength=1mm
	\begin{picture}(150,75)
	\put(10,0){\def\svgwidth{15cm}{\small\input{figures/bending_BVP.eps_tex}}}
	\end{picture}
	\caption{Bending boundary value problem. Inspection line can be seen in red.}
\end{figure} 

\begin{figure}[ht]
	\unitlength=1mm
         \includegraphics[width=0.75 \textwidth]{figures/deflection_traction.eps}
		  	\caption{Deflection curves along the line $y=0.5$ using different values of the characteristic length $L_c$.}
\end{figure} 


\begin{figure}[ht]
	\unitlength=1mm
	\center
		  	  \begin{subfigure}[b]{0.45\textwidth}
         \includegraphics[width=\textwidth]{figures/chi_h_lc=0,001.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=0.001$}
		  \end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
         \includegraphics[width=\textwidth]{figures/chi_h_lc=1.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1$}
		  \end{subfigure}
		  	  \begin{subfigure}[b]{0.45\textwidth}
         \includegraphics[width=\textwidth]{figures/chi_h_lc=1000.eps}
         \put(-35,-2){$x$}
	\caption{$L_c=1000$}
		  \end{subfigure}
		  	\caption{$\Bchi$  and $\Grad \bu$ components along the inspection line using different values of the characteristic length $L_c$.}
\end{figure} 

\begin{figure}[ht]
	\unitlength=1mm
         \includegraphics[width=0.75 \textwidth]{figures/potential_traction.eps}
		  	\caption{Potential of the relaxed micromorphic model along the inspection line using different values of the characteristic length $L_c$.}
\end{figure} 

\FloatBarrier
%=========================================================================
\sect{\hspace{-5mm}. Conclusion}
\vspace{-4mm}
%=========================================================================

\vspace{5cm}



